Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Monte Carlo

Riemannian manifold Hamiltonian Monte Carlo is traditionally carried out using the generalized leapfrog integrator. However, this integrator is not the only choice and other integrators yielding valid Markov chain transition operators may be considered. In this work, we examine the implicit midpoint integrator as an alternative to the generalized leapfrog integrator. We discuss advantages and disadvantages of the implicit midpoint integrator for Hamiltonian Monte Carlo, its theoretical properties, and an empirical assessment of the critical attributes of such an integrator for Hamiltonian Monte Carlo: energy conservation, volume preservation, and reversibility. Empirically, we find that while leapfrog iterations are faster, the implicit midpoint integrator has better energy conservation, leading to higher acceptance rates, as well as better conservation of volume and better reversibility, arguably yielding a more accurate sampling procedure.

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/algorithms/fixed-point-solver.tex <==
\begin{algorithm}[t!]
\caption{{\bf (Fixed Point Iteration)} Procedure for solving the equation $z=f(z)$ via fixed point interation to a given tolerance.}
\label{alg:fixed-point-solver}
\begin{algorithmic}[1]
\STATE \textbf{Input}: Function $f :\R^m\to\R^m$, initial guess $z\in\R^m$, fixed point convergence tolerance $\delta \geq 0$.
\STATE Set $\Delta z = \infty$ and $z' = z$.
\STATE \textbf{While}: $\Delta z > \delta$ compute
\begin{align}
    z'' &= f(z') \\
    \Delta z &= \max_{i\in\set{1,\ldots, m}} \abs{z''_i - z'_i} \\
    z' &= z''
\end{align}
\STATE \textbf{Return}: $z'\in\R^m$.
\end{algorithmic}
\end{algorithm}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/algorithms/generalized-leapfrog.tex <==
\begin{algorithm}[t!]
\caption{{\bf (G.L.F.(a))} The procedure for a single step of integrating Hamiltonian dynamics using the generalized leapfrog integrator.}
\label{alg:generalized-leapfrog}
\begin{algorithmic}[1]
\STATE \textbf{Input}: Hamiltonian $H:\R^m\times\R^m\to \R$, initial position and momentum variables $(q,p)\in\R^m\times\R^m$, integration step-size size $\epsilon\in\R$, fixed-point convergence tolerance $\delta \geq 0$.
\STATE Use \cref{alg:fixed-point-solver} with tolerance $\delta$ and initial guess $p$ to solve for $\bar{p}$,
% \STATE Solve the implicitly-defined equations for $\bar{p}$ to tolerance $\delta$,
\begin{align}
    \label{eq:glf-momentum-i} \bar{p} &\defeq \underbrace{p -\frac{\epsilon}{2} \nabla_q H(q, \bar{p})}_{f(\bar{p})}
\end{align}
\STATE Use \cref{alg:fixed-point-solver} with tolerance $\delta$ and initial guess $q$ to solve for $q'$,
\begin{align}
     \label{eq:glf-position} q' &\defeq \underbrace{q + \frac{\epsilon}{2} \paren{\nabla_p H(q, \bar{p}) + \nabla_p H(q', \bar{p})}}_{f(q')}
\end{align}
\STATE Compute the explicit update
\begin{align}
    \label{eq:glf-momentum-ii} p' &\defeq \bar{p} -\frac{\epsilon}{2} \nabla_qH(q', \bar{p})
\end{align}
\STATE \textbf{Return}: $(q', p')\in\R^m\times\R^m$.
\end{algorithmic}
\end{algorithm}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/algorithms/implicit-midpoint.tex <==
\begin{algorithm}[t!]
\caption{{\bf (I.M.(a))} The procedure for a single step of integrating Hamiltonian dynamics using the implicit midpoint integrator.}
\label{alg:implicit-midpoint}
\begin{algorithmic}[1]
\STATE \textbf{Input}: Hamiltonian $H:\R^m\times\R^m\to \R$, initial position and momentum variables $(q,p)\in\R^m\times\R^m$, integration step-size size $\epsilon\in\R$, fixed-point convergence tolerance $\delta \geq 0$.
\STATE Use \cref{alg:fixed-point-solver} with tolerance $\delta$ and initial guess $(q, p)$ to solve for $(q', p')$
\begin{align}
    \label{eq:implicit-midpoint} \begin{pmatrix} q' \\ p' \end{pmatrix} \defeq \underbrace{\begin{pmatrix} q \\ p \end{pmatrix} + \epsilon \begin{pmatrix} \nabla_p H(\bar{q}, \bar{p}) \\ -\nabla_q H(\bar{q},\bar{p}) \end{pmatrix}}_{f(q', p')}
\end{align}
where $\bar{q} \defeq (q' + q) / 2$ and $\bar{p} \defeq (p'+p)/2$.
\STATE \textbf{Return}: $(q', p')\in\R^m\times\R^m$.
\end{algorithmic}
\end{algorithm}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/algorithms/smart-generalized-leapfrog.tex <==
\begin{algorithm}[b!]
\caption{{\bf (G.L.F.(b))} The procedure for a single step of integrating Hamiltonian dynamics using the efficient implementation of the generalized leapfrog integrator.}
\label{alg:smart-generalized-leapfrog}
\begin{algorithmic}[1]
\STATE \textbf{Input}: Log-posterior $\mathcal{L}:\R^m\to \R$, Riemannian metric $\mathbb{G}:\R^m\to\R^{m\times m}$, initial position and momentum variables $(q,p)\in\R^m\times\R^m$, integration step-size size $\epsilon\in\R$.
\STATE Precompute $\mathbb{G}^{-1}(q)$, $\frac{\partial}{\partial q_i}\mathbb{G}(q)$, and define
\begin{align}
    A_i \defeq \frac{\partial}{\partial q_i} \mathcal{L}(q) + \frac{1}{2}\mathrm{trace}\paren{\mathbb{G}^{-1}(q) \frac{\partial}{\partial q_i}\mathbb{G}(q)}
\end{align}
for $i=1,\ldots, m$.
\STATE Use \cref{alg:fixed-point-solver} with tolerance $\delta$ and initial guess $p$ to solve for $\bar{p}$,
\begin{align}
    \label{eq:smart-generalized-leapfrog-momentum} \bar{p} &= \underbrace{p - \frac{\epsilon}{2}\paren{A_1 - \frac{1}{2} (\mathbb{G}^{-1}(q) \bar{p})^\top \frac{\partial}{\partial q_1}\mathbb{G}(q) (\mathbb{G}^{-1}(q) \bar{p}), \ldots, A_m - \frac{1}{2} (\mathbb{G}^{-1}(q) \bar{p})^\top \frac{\partial}{\partial q_m}\mathbb{G}(q) (\mathbb{G}^{-1}(q) \bar{p})}^\top}_{f(\bar{p})}.
\end{align}
\STATE Precompute $\mathbb{G}(q)^{-1}\bar{p}$.
\STATE Use \cref{alg:fixed-point-solver} with tolerance $\delta$ and initial guess $q$ to solve for $q'$,
\begin{align}
    \label{eq:smart-generalized-leapfrog-position} q' = \underbrace{q + \frac{\epsilon}{2}\paren{\mathbb{G}^{-1}(q)\bar{p} + \mathbb{G}^{-1}(q')\bar{p}}}_{f(q')}.
\end{align}
\STATE Compute $p'$ using \cref{eq:glf-momentum-ii}, which is an explicit update.
\STATE \textbf{Return}: $(q', p')\in\R^m\times\R^m$.
\end{algorithmic}
\end{algorithm}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/algorithms/smart-implicit-midpoint.tex <==
\begin{algorithm}[t!]
\caption{{\bf (I.M.(b))} The procedure for a single step of integrating Hamiltonian dynamics using the implicit midpoint integrator as advocated by \citet{leimkuhler_reich_2005}.}
\label{alg:smart-implicit-midpoint}
\begin{algorithmic}[1]
\STATE \textbf{Input}: Hamiltonian $H:\R^m\times\R^m\to \R$, initial position and momentum variables $(q,p)\in\R^m\times\R^m$, integration step-size size $\epsilon\in\R$, fixed-point convergence tolerance $\delta\geq 0$.
\STATE Use \cref{alg:fixed-point-solver} with tolerance $\delta$ and initial guess $(q, p)$ to solve for $(\bar{q},\bar{p})$, \begin{align}
    \label{eq:implicit-midpoint-implicit} \begin{pmatrix} \bar{q} \\ \bar{p} \end{pmatrix} \defeq \underbrace{\begin{pmatrix} q \\ p \end{pmatrix} + \frac{\epsilon}{2} \begin{pmatrix} \nabla_p H(\bar{q}, \bar{p}) \\ -\nabla_q H(\bar{q},\bar{p}) \end{pmatrix}}_{f(\bar{q},\bar{p})}.
\end{align}
\STATE Compute the explicit update
\begin{align}
    \label{eq:implicit-midpoint-explicit} \begin{pmatrix} q' \\ p' \end{pmatrix} =  \begin{pmatrix} \bar{q} \\ \bar{p} \end{pmatrix} + \frac{\epsilon}{2} \begin{pmatrix} \nabla_p H(\bar{q}, \bar{p}) \\ -\nabla_q H(\bar{q},\bar{p}) \end{pmatrix}.
\end{align}
\STATE \textbf{Return}: $(q', p')\in\R^m\times\R^m$.
\end{algorithmic}
\end{algorithm}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/detailed-balance.tex <==
\newpage
\section{Detailed Balance from Reversibility and Volume Preservation}\label{app:detailed-balance}

Let $\Phi : \R^{m}\times\R^m\to\R^m\times \R^m$ be a numerical integrator satisfying the following two properties as described in the main text:
\begin{enumerate}[(i)]
    \item The integrator has a unit Jacobian determinant so that it preserves volume in $(q, p)$-space.
    \item The integrator is symmetric under negation of the momentum variable.
\end{enumerate}

Given $(q, p)\in\R^m\times\R^m$, define the {\it momentum flip operator} by $\Psi(q, p) = (q, -p)$. For Markov chain Monte Carlo, we then define the Markov chain {\it proposal} operator by $\mathfrak{P} \defeq \Psi\circ\Phi$; because $\Phi$ satisfies property (ii) we have that $\mathfrak{P}\circ \mathfrak{P} = \Psi\circ\Phi \circ \Psi\circ\Phi = \mathrm{Id}$ so that the proposal operator is self-inverse $\mathfrak{P}^{-1} = \mathfrak{P}$. Moreover, $\Psi$ has unit Jacobian determinant: $\left|\mathrm{det}(\nabla\Psi)\right| = 1$; therefore, since $\Phi$ has unit Jacobian determinant by property (i), $\mathfrak{P}$ also has unit Jacobian determinant:
\begin{align}
    \left|\mathrm{det}(\nabla\mathfrak{P}(q, p)) \right| &= \left|\mathrm{det}(\nabla \Psi (\Phi(q, p)) \nabla \Phi(q, p))\right| \\
    &= \left|\mathrm{det}(\nabla \Psi (\Phi(q, p)) \cdot \mathrm{det}(\nabla \Phi(q, p))\right| \\
    &= 1
\end{align}

Given a current position $(q, p)$ of the Markov chain, the proposal for the next state of the Markov chain $(q',p') \defeq \mathfrak{P}(q, p)$ is accepted with probability
\begin{align}
    \min\set{1, \frac{\pi(q',p')}{\pi(q, p)}},
\end{align}
where $\pi:\R^m\times\R^m\to\R$ is the target distribution. (Notice that $\pi$ must only be specified up to a constant.) Thus, the Markov chain {\it transition} operator is defined by,
\begin{align}
    \mathfrak{T}(q, p) = \begin{cases}
    (q', p') & \mathrm{w.p.}~ \min\set{1, \frac{\pi(q',p')}{\pi(q, p)}} \\
    (q, p) & \mathrm{else}.
    \end{cases}
\end{align}

We say that detailed balance holds if for all sets $A, B\subset\R^m\times\R^m$ we have,
\begin{align}
    \underset{(q, p)\sim \pi}{\mathrm{Pr}}\left[(q,p)\in A ~\mathrm{and}~ \mathfrak{T}(q, p)\in B\right] = \underset{(q, p)\sim \pi}{\mathrm{Pr}}\left[(q,p)\in B ~\mathrm{and}~ \mathfrak{T}(q, p)\in A\right]
\end{align}
Let $z=(q, p)$. Expanding we compute,
\begin{align}
    \underset{z\sim \pi}{\mathrm{Pr}}\left[z\in A ~\mathrm{and}~ \mathfrak{T}(z)\in B\right] &= \int_A \pi(z) \cdot \mathbf{1}\set{\mathfrak{P}(z) \in B}\cdot \min\set{1, \frac{\pi(\mathfrak{P}(z))}{\pi(z)}}~\mathrm{d}z \\
    &= \int_{A\cap \mathfrak{P}(B)} \pi(z) \cdot \min\set{1, \frac{\pi(\mathfrak{P}(z))}{\pi(z)}}~\mathrm{d}z \\
    &\overset{z' = \mathfrak{P}(z)}{=} \int_{\mathfrak{P}(A)\cap B} \pi(\mathfrak{P}(z')) \cdot \min\set{1, \frac{\pi(z')}{\pi(\mathfrak{P}(z'))}}~\mathrm{d}z' \label{eq:change-of-variables} \\
    &= \int_{\mathfrak{P}(A)\cap B} \pi(z')  \cdot \min\set{1, \frac{\pi(\mathfrak{P}(z'))}{\pi(z')}}~\mathrm{d}z' \\
    &= \int_{B} \pi(z') \cdot \mathbf{1}\set{\mathfrak{P}(z')\in A}  \cdot \min\set{1, \frac{\pi(\mathfrak{P}(z'))}{\pi(z')}}~\mathrm{d}z' \\
    &= \underset{z\sim \pi}{\mathrm{Pr}}\left[z\in B ~\mathrm{and}~ \mathfrak{T}(z)\in A\right]
\end{align}
showing that detailed balance holds. The change-of-variables in \cref{eq:change-of-variables} does not incur a Jacobian determinant correction since $\mathfrak{P}$ has unit Jacobian determinant.


==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/experiment-logistic-regression.tex <==
\newpage
\section{Bayesian Logistic Regression}\label{app:experiment-bayesian-logistic-regression}



Binary classification is a uniquitous task in the data sciences and logistic regression is the most popular algorithm for obtaining probabilistic estimates of class membership. Bayesian logistic regression simply equips each of the linear coefficients in the logistic regression model with a prior distribution. We consider Bayesian logistic regression as defined by the following generative model:
\begin{align}
    y_i \vert x_i,\beta  &\sim\mathrm{Bernoulli}(\sigma(x_i^\top\beta)) ~~~~~~~\mathrm{for}~ i=1,\ldots,n  \\
    \beta_i &\sim \mathrm{Normal}(0, 1) ~~~~~~~~~~~~~~~\mathrm{for}~ i=1,\ldots,k,
\end{align}
where $x_i\in \R^k$ is vector of explanatory variables and $\sigma :\R\to (0,1)$ is the sigmoid function. For the logistic regression model, let $\mathbf{x}\in\R^{n\times m}$ represent the matrix of features. The Riemannian metric formed by the sum of the Fisher information and the negative Hessian of the log-prior is $\mathbb{G}(\beta) = \mathbf{x}^\top \boldsymbol{\Lambda}\mathbf{x} + \mathrm{Id}$ where $\boldsymbol{\Lambda}$ is a diagonal matrix whose $i^\text{th}$ diagonal entry is $\sigma(x_i^\top \beta) (1-\sigma(x_i^\top \beta))$.


We consider sampling from the posterior distribution of the linear coefficients for a breast cancer, heart disease, and diabetes dataset. We consider integration step-sizes in $\set{1/10, 1}$ and a number of integration steps in $\set{5, 10, 50}$; each configuration of step-size and number of steps is replicated ten times and we attempt to draw 10,000 samples from the posterior. Results are presented in \cref{tab:logistic-regression-breast-cancer,tab:logistic-regression-diabetes,tab:logistic-regression-heart}. For the smaller step-size, both integrators enjoy very high acceptance rates and similar performance when {\it not} adjusted for timing; when adjusted for timing, the generalized leapfrog is often the better choice in the presence of a small step-size. For the larger step-size, only the implicit midpoint integrator is able to maintain a high acceptance rate; occasionally, the implicit midpoint is able to produce the optimal mean ESS and minimum ESS {\it per second}.

\clearpage
\input{tables/logistic-regression-breast-cancer}
\input{tables/logistic-regression-diabetes}
\input{tables/logistic-regression-heart}
\clearpage

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/experiment-quadratic-hamiltonian.tex <==
\newpage
\section{Quadratic Hamiltonian}\label{app:experiment-quadratic-hamiltonian}

\input{figures/gaussian-energy}

We consider using HMC to draw samples from a Gaussian distribution in two dimensions. In particular, we aim to sample from the joint distribution of position and momentum defined by,
\begin{align}
    q&\sim \mathrm{Normal}\paren{\begin{pmatrix} 1/2 \\ -1 \end{pmatrix}, \begin{pmatrix} 1 & 1/2 \\ 1/2 & 2 \end{pmatrix}} \\
    p&\sim \mathrm{Normal}\paren{\begin{pmatrix} 0 \\ 0 \end{pmatrix}, \begin{pmatrix} 1 & 1/2 \\ 1/2 & 2 \end{pmatrix}^{-1}}
\end{align}
These distributions correspond to the quadratic Hamiltonian $H(q, p)=\frac{1}{2} q^\top \Sigma^{-1} q + \frac{1}{2} p^\top\Sigma p$. This Hamiltonian can be interpreted in the Riemannian manifold setting as sampling from the posterior $q\sim\mathrm{Normal}(\mu,\Sigma)$ and the constant metric $\mathbb{G}(q) = \Sigma^{-1}$.
The corresponding Hamiltonian is quadratic and therefore \cref{thm:first-integral-implicit-midpoint} applies. We expect perfect conservation of the Hamiltonian regardless of step-size. To evaluate the conservation of the Hamiltonian energy, we consider drawing $(q, p)$ from their joint distribution and integrating Hamilton's equations of motion for ten integration steps. We consider integration step-sizes in $\set{0.01, 0.1, 1.0}$. We then compare the initial Hamiltonian energy to the Hamiltonian energy at the terminal point of the integrator. We repeat this procedure 10,000 times and show the results in \cref{fig:gaussian-energy}, where the absolute difference in Hamiltonian energy is shown as a histogram. This experiment clearly shows that the implicit midpoint integrator has excellent conservation of the quadratic Hamiltonian energy and is orders of magnitude better than the generalized leapfrog integrator. Note that for a separable Hamiltonian, as is the case here, the steps of the generalized leapfrog integrator reduce to the standard leapfrog method.

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/fixed-point-iteration.tex <==
\newpage
\section{Implementation of Integrators}\label{app:implementation-of-integrators}


\subsection{Implementations of the Generalized Leapfrog Integrator}

As the purpose of this research is to compare two integrators for Hamiltonian Monte Carlo, we wish to be precise about how these numerical methods have been implemented. 

\input{algorithms/smart-generalized-leapfrog}

The first implementation of the generalized leapfrog integrator is presented in \cref{alg:generalized-leapfrog}. 
The system \cref{eq:glf-momentum-i,eq:glf-position,eq:glf-momentum-ii} was described as ``naive'' because it appears to ignore important structural properties of the equations of motion in \cref{eq:position-evolution,eq:momentum-evolution} that would accelerate a step of the generalized leapfrog integrator. For instance, in \cref{eq:glf-momentum-i}, the metric $\mathbb{G}(q)$ may be precomputed because it is an invariant of the fixed-point relation. Another example is that $\mathbb{G}^{-1}(q)\bar{p}$ is an invariant quantity of \cref{eq:glf-position} and need not be recomputed in each fixed-point iteration. Thus, we see that the generalized leapfrog integrator, when efficiently implemented, has an important computational advantage in that certain invariant quantities can be ``cached'' when finding fixed points. A more complicated implementation of the generalized leapfrog integrator with caching is presented in given in \cref{alg:smart-generalized-leapfrog}. We stress that \cref{alg:generalized-leapfrog,alg:smart-generalized-leapfrog} perform the same calculation.

\subsection{Implementations of the Implicit Midpoint Integrator}

\input{algorithms/smart-implicit-midpoint}

In addition to the implementation of the implicit midpoint method described in \cref{alg:implicit-midpoint}, we also consider a variant advocated by \citet{leimkuhler_reich_2005} and present the implementation in \cref{alg:smart-implicit-midpoint}. The essential difference between \cref{alg:implicit-midpoint,alg:smart-implicit-midpoint} is whether or not the implicitly-defined update computes the terminal point of the step (\cref{alg:implicit-midpoint}) or the midpoint of the step (\cref{alg:smart-implicit-midpoint}). We stress that \cref{alg:implicit-midpoint,alg:smart-implicit-midpoint} perform the same calculation when $\delta=0$, which is easily verified by plugging \cref{eq:implicit-midpoint-implicit} into \cref{eq:implicit-midpoint-explicit} and comparing to \cref{eq:implicit-midpoint}. Unlike the generalized leapfrog integrator, the implicit midpoint integrator does not enjoy the ability to cache intermediate computations.

\subsection{Remarks on Computational Complexity}\label{app:lipschitz-fixed-point}

In discussing the computational complexity of the generalized leapfrog and implicit midpoint methods, we will assume that the functions defining the fixed-point relations are {\it contraction maps}. Contraction maps in a complete metric space guarantee that fixed point equations have unique solutions and that these solutions are reached via fixed point iteration for any initial condition. Moreover, contraction maps have known convergence rates, which are convenient for analysis.

\begin{definition}
The $L_\infty$ distance on $\R^m$ is defined by
\begin{align}
    d_\infty(z, z') \defeq \max_{i=1,\ldots, m} \abs{z_i - z'_i}.
\end{align}
\end{definition}
We will restrict our attention to the $L_\infty$ distance as it is used as our convergence criterion in \cref{alg:fixed-point-solver}.
\begin{definition}
A contraction map on $\R^m$ is a Lipschitz function $f:\R^m\to\R^m$ whose Lipschitz constant is less than one; that is,
\begin{align}
   d_\infty(f(z), f(z')) \leq L \cdot d_\infty(z, z')
\end{align}
for all $z, z'\in\R^m$ and where $L\in [0, 1)$.
\end{definition}


\begin{theorem}[Banach Fixed Point Theorem]
Let $f :\R^m\to\R^m$ be a contraction map with Lipschitz constant $L\in [0, 1)$. Then (i) the equation $z=f(z)$ has a unique solution; (ii) the fixed point iterations $z_{n+1} = f(z_n)$ converge to $z$ from any $z_0\in\R^m$; (iii) the distance between iterates satisfies $d_\infty(z_{n+1},z_n) \leq L^n d_\infty(z_1, z_0)$.
\end{theorem}

In assessing convergence to the unique solution using fixed point iteration, \cref{alg:fixed-point-solver} demands that $d_\infty(z_{n+1},z_n) \leq \delta$ for some convergence tolerance $\delta >0$. Assuming that $d_\infty(z_1, z_0) > 0$, we can rearrange $L^n d_\infty(z_1, z_0) \leq \delta$ to give a sufficient condition on the number of fixed point iterates $n$ to guarantee that $d_\infty(z_{n+1},z_n) \leq \delta$. Namely:
\begin{lemma}
Assume $d_\infty(z_1, z_0) > 0$. Then the choice
\begin{align}
    n = \ceil[\Bigg]{\frac{\log \delta - \log d_\infty(z_1, z_0)}{\log L}}
\end{align}
is sufficient to ensure that $d_\infty(z_{n+1},z_n) \leq \delta$.
\end{lemma}
\begin{proof}
From the Banach fixed point theorem we know that $d_\infty(z_{n+1},z_n) \leq L^n d_\infty(z_1, z_0)$. Therefore, we seek to establish when the right-hand side of the inequality is less than $\delta$. Rearranging and noting that $\log L$ is negative (since $f$ is a contraction map) yields
\begin{align}
    n \geq \frac{\log \delta - \log d_\infty(z_1, z_0)}{\log L}.
\end{align}
It makes sense to use the smallest integer $n$ such that the $d_\infty(z_{n+1},z_n) \leq \delta$ so computing the ceiling of the right-hand side yields the result.
\end{proof}

Under the assumption that functions defining fixed point equations are contractions, we can give an approximate comparison of the computational complexity of the implicit midpoint and generalized leapfrog algorithms. In integrating the dynamics corresponding to a Hamiltonian as in \cref{eq:hamiltonian-energy} (refer to \cref{eq:position-evolution,eq:momentum-evolution}), there are several operations of notable computational complexity; these are (i) computing the gradient of the log-likelihood, (ii) computing the inverse of the Riemannian metric, and (iii) computing the derivatives of the Riemannian metric. To make this slightly more formal, let $\mathrm{Cost}(\nabla \mathcal{L})$, $\mathrm{Cost}(\mathbb{G}^{-1})$, and $\mathrm{Cost}(\nabla \mathbb{G})$ denote some notion of computational complexity associated to these three quantities; we assume that any remaining arithmetic operations used in the integration of Hamilton's mechanics have negligible computational cost.

\begin{example}
For the implicit midpoint integrator, each of the above quantities (i)-(iii) must be computed within each fixed point iteration. If $L_\mathrm{imp}$ denotes the Lipschitz constant associated to the map $f$ in \cref{eq:implicit-midpoint}, then the total computational cost of the implicit midpoint integrator is
\begin{align}
    \label{eq:cost-implicit-midpoint} \ceil[\Bigg]{\frac{\log \delta - \log d_\infty(f(z_0), z_0)}{\log L_\mathrm{imp}}} \cdot \paren{\mathrm{Cost}(\nabla \mathcal{L}) + \mathrm{Cost}(\mathbb{G}^{-1}) + \mathrm{Cost}(\nabla \mathbb{G})}.
\end{align}
\end{example}
\begin{example}
The situation is rather different for the generalized leapfrog integrator as expressed in \cref{alg:smart-generalized-leapfrog}. The fixed point equation in \cref{eq:smart-generalized-leapfrog-momentum} requires that we compute quantities (i)-(iii); however, these are invariant of the fixed point equation in \cref{eq:smart-generalized-leapfrog-momentum}, which therefore does not incur additional cost beyond the sum of $\mathrm{Cost}(\nabla \mathcal{L})$, $\mathrm{Cost}(\mathbb{G}^{-1})$, and $\mathrm{Cost}(\nabla \mathbb{G})$. For the second fixed point equation, let $L_\mathrm{glf}$ denote the Lipschitz constant of the contraction map $f$ in \cref{eq:smart-generalized-leapfrog-position}; each iteration requires computing the inverse of the Riemannian metric. Thus, the computational cost incurred by the second fixed point equation is
\begin{align}
    \ceil[\Bigg]{\frac{\log \delta - \log d_\infty(f(q_0), q_0)}{\log L_\mathrm{glf}}} \cdot \mathrm{Cost}(\mathbb{G}^{-1}).
\end{align}
The final step of the generalized leapfrog integrator requires an explicit update wherein we compute quantities (i)-(iii) using the updated position variable. In total, the cost of a step of the generalized leapfrog integrator is therefore,
\begin{align}
    \label{eq:cost-generalized-leapfrog} \ceil[\Bigg]{\frac{\log \delta - \log d_\infty(f(q_0), q_0)}{\log L_\mathrm{glf}}} \cdot \mathrm{Cost}(\mathbb{G}^{-1}) + 2\cdot \paren{\mathrm{Cost}(\nabla \mathcal{L}) + \mathrm{Cost}(\mathbb{G}^{-1}) + \mathrm{Cost}(\nabla \mathbb{G})}.
\end{align}
\end{example}

\subsection{Counts of Fixed Point Iterations}

\input{figures/banana-fixed-point}
\input{figures/stochastic-volatility-fixed-point}
\input{figures/fitzhugh-nagumo-fixed-point}

In this section we compute the number of fixed point iterations performed by both the implicit midpoint and generalized leapfrog integrators on the banana, stochastic volatility, and Fitzhugh-Nagumo experiments.  We report the relative frequency of each number of the fixed point iterations over the course of sampling. We note that this is for context only, and that the precise number of fixed point iterations consumed by either integrator are not comparable to one another; the reason for this is that the amount of computation differs for the implicit midpoint and generalized leapfrog methods as described in \cref{app:lipschitz-fixed-point}. For the generalized leapfrog method, we report the total number of iterations to solve both fixed point relations to the prescribed tolerance. Results are shown in \cref{fig:stochastic-volatility-fixed-point,fig:fitzhugh-nagumo-fixed-point,fig:banana-fixed-point} for a convergence tolerance of $\delta = 1\times 10^{-6}$.

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/implicit-midpoint-eigenvalues.tex <==
\newpage
\section{Implicit Midpoint Eigenvalues}\label{app:implicit-midpoint-eigenvalues}

Let $z=(q,p)$ and consider a quadratic Hamiltonian of the form,
\begin{align}
    H(z) &= z^\top \mathbf{A}z \\
    &= \begin{pmatrix} q^\top & p^\top \end{pmatrix} \begin{pmatrix} \Sigma & 0 \\ 0 & \Sigma \end{pmatrix} \begin{pmatrix} q \\ p \end{pmatrix}.
\end{align}
The associated Hamiltonian vector field is,
\begin{align}
    \dot{z} &= \begin{pmatrix} \dot{q} \\ \dot{p} \end{pmatrix} \\
    &= \begin{pmatrix} 0 & \mathrm{Id} \\ -\mathrm{Id} & 0 \end{pmatrix} \begin{pmatrix} \Sigma & 0 \\ 0 & \Sigma \end{pmatrix} \begin{pmatrix} q \\ p \end{pmatrix} \\
    &= \underbrace{\begin{pmatrix} 0 & \Sigma \\ -\Sigma & 0 \end{pmatrix}}_{\mathbf{J}} \begin{pmatrix} q \\ p \end{pmatrix} \\
    &= \mathbf{J}z.
\end{align}

From \cref{eq:implicit-midpoint}, the implicit midpoint integrator computes the update,
\begin{align}
    & z' = z + \epsilon \mathbf{J}\paren{\frac{z' + z}{2}} \\
    \implies & z' = z + \frac{\epsilon}{2}\mathbf{J}z' + \frac{\epsilon}{2}\mathbf{J}z \\
    \implies& \paren{\mathrm{Id} - \frac{\epsilon}{2}\mathbf{J}}z' = \paren{\mathrm{Id} + \frac{\epsilon}{2}\mathbf{J}}z \\
    \implies& z' = \underbrace{\paren{\mathrm{Id} - \frac{\epsilon}{2}\mathbf{J}}^{-1}\paren{\mathrm{Id} + \frac{\epsilon}{2}\mathbf{J}}}_{\mathbf{Q}}z
\end{align}
The quantity $\mathbf{Q}$ is the Cayley transform of the linear transformation $\frac{\epsilon}{2}\mathbf{J}$. Noting that $\mathbf{J}$ is a skew-symmetric matrix, it is an established fact that the Cayley transform of a skew-symmetric matrix is an orthogonal matrix. This establishes that all of the eigenvalues of $\mathbf{Q}$, the linear transform representing the implicit midpoint integrator, have unit modulus.

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/implicit-midpoint-symmetry.tex <==
\newpage
\section{Momentum Negation Symmetry of Implicit Midpoint}\label{app:momentum-negation-implicit-midpoint}

\begin{lemma}\label{lem:implicit-midpoint-momentum-flip}
Given a Hamiltonian $H$ in the form of \cref{eq:hamiltonian-energy}, step-size $\epsilon$, and initial position $(q, p)$, compute $(q', p')$ according to \cref{alg:implicit-midpoint} with $\delta=0$. If one then computes $(q'', p'')$ from initial position $(q', -p')$ using \cref{alg:implicit-midpoint} a second time (with the same Hamiltonian, step-size, and $\delta=0$), then $q''=q$ and $-p'' = p$.
\end{lemma}
\Cref{lem:implicit-midpoint-momentum-flip} establishes that the implicit midpoint integrator is suitable for HMC in that it satisfies properties (i) and (ii).

\begin{proof}
Consider the initial condition $(q, p)$ and a fixed step-size of $\epsilon$. For the Riemannian manifold Hamiltonian Monte Carlo, the implicit midpoint integrator computes the following updates:
\begin{align}
    \label{eq:implicit-reverse-position} q'_i &= q_i + \epsilon\paren{\sum_{j=1}^m \mathbb{G}^{-1}_{ij}\paren{\frac{q' + q}{2}}\paren{\frac{p'_j + p_j}{2}}} \\
    \label{eq:implicit-reverse-momentum} \begin{split}
    p'_i &= p_i + \epsilon\left(-\frac{\partial}{\partial q_i}\mathcal{L}\paren{\frac{q' + q}{2}} - \frac{1}{2} \mathrm{trace}\paren{\mathbb{G}^{-1}\paren{\frac{q' + q}{2}} \frac{\partial}{\partial q_i} \mathbb{G}\paren{\frac{q' + q}{2}}} + \right.\\
    &\qquad \left.\frac{1}{2} \paren{\frac{p' + p}{2}}^\top\mathbb{G}^{-1}\paren{\frac{q' + q}{2}} \frac{\partial}{\partial q_i}\mathbb{G}\paren{\frac{q' + q}{2}} \mathbb{G}^{-1}\paren{\frac{q' + q}{2}} \paren{\frac{p' + p}{2}}\right)
    \end{split}
\end{align}
What we want to show is that if we compute $(q', p')$, negate the momentum $(q', p')\mapsto (q', -p')$, and apply the implicit midpoint integrator a second time, then we arrive at $(q, -p)$. Thus, we need to establish that $(q, -p)$ is a fixed point of the relations,
\begin{align}
    q''_i &= q'_i + \epsilon\paren{\sum_{j=1}^m \mathbb{G}^{-1}_{ij}\paren{\frac{q'' + q'}{2}}\paren{\frac{p''_j + (-p_j')}{2}}} \\
    \begin{split}
    p''_i &= -p'_i + \epsilon\left(-\frac{\partial}{\partial q_i}\mathcal{L}\paren{\frac{q'' + q'}{2}} - \frac{1}{2} \mathrm{trace}\paren{\mathbb{G}^{-1}\paren{\frac{q'' + q'}{2}} \frac{\partial}{\partial q_i} \mathbb{G}\paren{\frac{q'' + q'}{2}}} + \right.\\
    &\qquad \left.\frac{1}{2} \paren{\frac{p'' + (-p')}{2}}^\top\mathbb{G}^{-1}\paren{\frac{q'' + q'}{2}} \frac{\partial}{\partial q_i}\mathbb{G}\paren{\frac{q'' + q'}{2}} \mathbb{G}^{-1}\paren{\frac{q'' + q'}{2}} \paren{\frac{p'' + (-p')}{2}}\right).
    \end{split}
\end{align}
Plugging in we obtain,
\begin{align}
    q'_i + \epsilon\paren{\sum_{j=1}^m \mathbb{G}^{-1}_{ij}\paren{\frac{q + q'}{2}}\paren{\frac{(-p_j) + (-p_j')}{2}}} &= q'_i - \epsilon\paren{\sum_{j=1}^m \mathbb{G}^{-1}_{ij}\paren{\frac{q + q'}{2}}\paren{\frac{p_j + p_j'}{2}}} \\
    &= q_i
\end{align}
by rearranging \cref{eq:implicit-reverse-position}. For notational simplicity let us define
\begin{align}
    U\paren{q} &\defeq -\frac{\partial}{\partial q_i}\mathcal{L}\paren{q} - \frac{1}{2} \mathrm{trace}\paren{\mathbb{G}^{-1}\paren{q} \frac{\partial}{\partial q_i} \mathbb{G}\paren{q}} \\
    R\paren{q} &\defeq \frac{1}{2}\mathbb{G}^{-1}\paren{q} \frac{\partial}{\partial q_i}\mathbb{G}\paren{q} \mathbb{G}^{-1}\paren{q}
\end{align}
so that
\begin{align}
    p''_i = -p'_i + \epsilon \paren{U\paren{\frac{q'' + q}{2}} + \paren{\frac{p'' + (-p')}{2}}^\top R\paren{\frac{q'' + q}{2}}\paren{\frac{p'' + (-p')}{2}}}.
\end{align}
Plugging in, we obtain,
\begin{align}
    & -p'_i + \epsilon \paren{U\paren{\frac{q + q}{2}} + \paren{\frac{(-p) + (-p')}{2}}^\top R\paren{\frac{q + q}{2}}\paren{\frac{(-p) + (-p')}{2}}} \\
    =& -p'_i + \epsilon \paren{U\paren{\frac{q + q}{2}} + \paren{\frac{p + p'}{2}}^\top R\paren{\frac{q + q}{2}}\paren{\frac{p + p'}{2}}} \\
    =& -p_i
\end{align}
which follows from negating \cref{eq:implicit-reverse-momentum} and rearranging.
\end{proof}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/numerical-stability.tex <==
\newpage
\section{Numerical Stability}\label{app:numerical-stability}

The stability of numerical integrators is defined by their long-term behavior on the harmonic oscillator, which is described by the following Hamiltonian system
\begin{align}
    \dot{q} = p ~~~~~~~~~~~~~~~ \dot{p} = -\omega^2 q,
\end{align}
corresponding to the Hamiltonian $H(q, p) = \omega^2 \frac{q^2}{2} + \frac{p^2}{2}$ where $\omega^2$ is a constant. Consider a single step of a numerical integrator for the harmonic oscillator with step-size $\epsilon$ that maps $(q, p)\mapsto (q', p')$. Because the harmonic oscillator is a {\it linear} differential equation, it is often possible find a matrix $\mathbf{R}\in\R^{2\times 2}$ such that $(q',p')^\top = \mathbf{R}(q,p)^\top$. A numerical method is called {\it stable} if the eigenvalues of $\mathbf{R}$ lie on the unit disk of the complex plane and are not repeated \cite{leimkuhler_reich_2005}. We have the following result.
\begin{proposition}\label{prop:implicit-midpoint-eigenvalues}
When $\epsilon < 2 / \omega$, the (generalized) leapfrog integrator is stable. The implicit midpoint integrator is stable for any $\epsilon$.
\end{proposition}
See \citet{leimkuhler_reich_2005,Hairer:1250576} for an introduction to stability analysis of numerical integrators.

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/proof-implicit-hmc.tex <==
\clearpage
\section{Proof of \Cref{prop:implicit-midpoint-quadratic-hamiltonian}}\label{app:implicit-midpoint-quadratic-hamiltonian}

\begin{proof}
The implicit midpoint integrator conserves quadratic first integrals (see \cref{thm:first-integral-implicit-midpoint}) and, in this case, the Hamiltonian energy is itself a quadratic function. 
\end{proof}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/randomized-step-design.tex <==
\clearpage
\section{Randomized Step Experimental Design}\label{app:randomized-step-experimental-design}


In the main text we have considered a grid search over the number of integration steps and use this number of steps in generating every proposal using either the implicit midpoint or generalized leapfrog integrators. An alternative experimental design is to randomize the number of integration steps for each proposal by sampling the number of steps uniformly between one and some upper bound. When the Hamiltonian is separable, the leapfrog integrator with a single step recovers the Metropolis-adjusted Langevin algorithm, which has known ergodicity properties. Therefore, it may be anticipated that randomizing the number of integration steps may lead to improved ergodicity when the proposal is computed by the generalized leapfrog method. In this appendix, we consider randomizing the number of integration steps for both the implicit midpoint and generalized leapfrog integrators.

\subsection{Banana-Shaped Distribution}

\input{tables/randomized-step-banana-ess}

Results for the banana-shaped distribution when using the randomized number of steps experimental design are presented in \cref{tab:randomized-step-banana-ess}.

\subsection{Neal Funnel}

\input{tables/randomized-step-neal-funnel-ess}

Results for Neal's funnel distribution when using the randomized number of steps experimental design are presented in \cref{tab:randomized-step-neal-funnel-ess}.


\subsection{Stochastic Volatility Model}

\input{tables/randomized-step-stochastic-volatility-symmetry-volume-preservation}

Results for the stochastic volatility model when using the randomized number of steps experimental design are presented in \cref{tab:randomized-step-stochastic-volatility-symmetry-volume-preservation}.


\subsection{Fitzhugh-Nagumo Differential Equation Model}

\input{tables/randomized-step-fitzhugh-nagumo}

Results for the Fitzhugh-Nagumo posterior when using the randomized number of steps experimental design are presented in \cref{tab:randomized-step-fitzhugh-nagumo-ess}.

\subsection{Bayesian Logistic Regression}

\input{tables/randomized-step-logistic-regression-breast-cancer}
\input{tables/randomized-step-logistic-regression-diabetes}
\input{tables/randomized-step-logistic-regression-heart}

Results for the Bayesian logistic regression models with a randomized number of steps are presented in \cref{tab:randomized-step-logistic-regression-breast-cancer,tab:randomized-step-logistic-regression-diabetes,tab:randomized-step-logistic-regression-heart}.

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/silent-change-of-variables.tex <==
\newpage
\section{Riemannian Metrics and a Silent Change-of-Variables?}


The Riemannian volume measure is $\sqrt{\mathrm{det}(\mathbb{G}(q))}~\mathrm{d}q$ on $\R^m$. When using HMC, does the fact that we have introduced a metric mean that we require a Jacobian correction to the posterior? Actually, the answer is no. The reason is that the Metropolis-Hastings accept-reject rule determines which density (specified with respect to the Lebesgue measure in the $(q, p)$ phase-space) is sampled by the Markov chain. Just because the acceptance Hamiltonian (which is also the guidance Hamiltonian in RMHMC; see \citet{Duane1987216}) involves computing the Riemannian metric does not mean that we have silently changed the underlying measure. Indeed, the log-determinant term appearing in \cref{eq:hamiltonian-energy} is chosen so that the conditional distribution of $p$ given $q$ is multivariate normal {\it with respect to the Lebesgue measure}.

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/appendices/volume-preservation-and-symmetry-metrics.tex <==
\newpage
\section{Volume Preservation and Symmetry Metrics}\label{app:volume-preservation-and-symmetric-metrics}

Here we describe how we compute metrics related to volume preservation and symmetry. Let $(q_1,\ldots, q_n)$ be samples generated by Hamiltonian Monte Carlo with numerical integrator $\Phi :\R^m\times\R^m\to\R^m\times\R^m$; each $q_i$ is an element of $\R^m$. 

\subsection{Reversibility}

For each sample $q_i$, generate $p_i\vert q_i \sim \mathrm{Normal}(0,\mathbb{G}(q_i))$ and compute $(q_i', p_i') = \Phi(q_i, p_i)$. Now compute $(q_i'', -p_i'') = \Phi(q_i', -p_i')$. The {\it violation of reversibility} is defined by
\begin{align}
    \sqrt{\Vert (q_i, p_i') - (q_i'', p_i'')\Vert_2^2}.
\end{align}
If the numerical integrator is reversible, this norm will be zero. In our metrics, we report the median violation of reversibility.

\subsection{Volume Preservation}

Let $z=(q, p)$ and identify $\Phi(z)\equiv \Phi(q, p)$. Define $f_j(z) = \frac{\Phi(z_1,\ldots, z_j + \eta / 2, \ldots, z_{2m}) - \Phi(z_1,\ldots, z_j - \eta / 2, \ldots, z_{2m})}{\eta}$ for $\eta = 1\times 10^{-5}$ (except for the Fitzhugh-Nagumo model where we set $\eta=1\times 10^{-3}$ for numerical reasons), which is the central difference formula that approximates $\frac{\partial}{\partial z_j} \Phi(z)$. We compute the approximation to the Jacobian of $\Phi$ by constructing,
\begin{align}
    \nabla \Phi(z) \approx F(z) \defeq \begin{pmatrix} f_1(z) & f_2(z) &\cdots & f_{2m}(z) \end{pmatrix} \in\R^{2m\times2m}.
\end{align}
For each sample $q_i$, generate $p_i\vert q_i \sim \mathrm{Normal}(0,\mathbb{G}(q_i))$ and set $z_i = (q_i, p_i)$. 
The {\it violation of volume preservation} is defined by
\begin{align}
    \left|\mathrm{det}(F(z_i)) - 1\right|.
\end{align}
If the numerical integrator is volume preserving, this difference will be zero.  In our metrics, we report the median violation of volume preservation.

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/figures/banana-fixed-point.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{images/banana-fixed-point.png}
    \caption{Visualization of the relative frequency of the number of fixed point iterations in the implicit midpoint and generalized leapfrog integration procedure for the banana-shaped distribution.}
    \label{fig:banana-fixed-point}
\end{figure*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/figures/banana-symmetry-volume-preservation.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/banana-reversibility-volume-step-size-0.1-num-steps-5-randomize-steps-False.png}
        \caption{$\epsilon=1/10$ and $5$ steps}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/banana-reversibility-volume-step-size-0.1-num-steps-10-randomize-steps-False.png}
        \caption{$\epsilon=1/10$ and $10$ steps}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/banana-reversibility-volume-step-size-0.1-num-steps-50-randomize-steps-False.png}
        \caption{$\epsilon=1/10$ and $50$ steps}
    \end{subfigure}
    \caption{Comparison between the error in symmetry and error in volume preservation properties of the implicit midpoint integrator and the generalized leapfrog integrator on the banana-shaped distribution. We observe that the implicit midpoint integrator tends to produce transitions whose median reversibility and volume preservation can be an order of magnitude, or more, better than the generalized leapfrog integrator. Each point is the median of one-hundred measurements of symmetry and reversibility shown for each of the ten trials. For $\epsilon=1/10$ and fifty integration steps, the generalized leapfrog integrator exhibits severely divergent behavior. {\bf The implicit midpoint is represented by the symbol $(\boldsymbol{\cdot})$ and the generalized leapfrog by the symbol $(+)$.}}
    \label{fig:banana-symmetry-volume-preservation}
\end{figure*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/figures/fitzhugh-nagumo-fixed-point.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{images/fitzhugh-nagumo-fixed-point.png}
    \caption{Visualization of the relative frequency of the number of fixed point iterations in the implicit midpoint and generalized leapfrog integration procedure for the Fitzhugh-Nagumo model.}
    \label{fig:fitzhugh-nagumo-fixed-point}
\end{figure*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/figures/fitzhugh-nagumo-symmetry-volume-preservation.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/fitzhugh-nagumo-reversibility-volume-step-size-1.0-num-steps-1-hmax-0.0.png}
        \caption{One integration step}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/fitzhugh-nagumo-reversibility-volume-step-size-1.0-num-steps-2-hmax-0.0.png}
        \caption{Two integration steps}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/fitzhugh-nagumo-reversibility-volume-step-size-1.0-num-steps-5-hmax-0.0.png}
        \caption{Five integration steps}
    \end{subfigure}
    \caption{Comparison of the degree to which the implicit midpoint and generalized leapfrog integrators violate reversibility and volume preservation on the Fitzhugh-Nagumo posterior. We observe that for the chosen convergence tolerances, the implicit midpoint integrator tends to exhibit better reversibility and volume preservation except for the smallest tolerance where the generalized leapfrog has slightly better volume preservation but worse reversibility. {\bf The implicit midpoint is represented by the symbol $(\boldsymbol{\cdot})$ and the generalized leapfrog by the symbol $(+)$.}}
    \label{fig:fitzhugh-nagumo-symmetry-volume}
\end{figure*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/figures/gaussian-energy.tex <==
\begin{figure*}[b!]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/gaussian-energy-conservation-step-size-0.01.png}
        \caption{$\epsilon=1/100$}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/gaussian-energy-conservation-step-size-0.1.png}
        \caption{$\epsilon=1/10$}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/gaussian-energy-conservation-step-size-1.0.png}
        \caption{$\epsilon=1$}
    \end{subfigure}
    \caption{Comparison between the energy conservation of the implicit midpoint integrator and the generalized leapfrog integrator on a quadratic Hamiltonian. We observe that for every step-size, the energy conservation of the implicit midpoint method is in the neighborhood of $1\times 10^{-10}$ whereas the generalized leapfrog has energy conservation that degrades with larger steps.}
    \label{fig:gaussian-energy}
\end{figure*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/figures/gaussian-stability-energy-conservation.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{images/gaussian-contour.png}
    \caption{Trajectories computed by the leapfrog integrator and the implicit midpoint integrator for a quadratic, separable Hamiltonian $H(q, p) = q^\top q / 2 + p^\top p / 2$. Both integrators are stable but the leapfrog integrator deviates from the level sets of the Hamiltonian (faint blue circles) whereas every iterate of the implicit midpoint integrator lies on the same energy level set as the previous one.}
    \label{fig:gaussian-stability-energy-conservation}
\end{figure}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/figures/neal-funnel-symmetry-volume-preservation.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/neal-funnel-reversibility-volume-step-size-0.1-num-steps-20.png}
        \caption{$\epsilon=1/10$}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/neal-funnel-reversibility-volume-step-size-0.2-num-steps-20.png}
        \caption{$\epsilon=1/5$}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/neal-funnel-reversibility-volume-step-size-0.5-num-steps-20.png}
        \caption{$\epsilon=1/2$}
    \end{subfigure}
    \caption{Comparison of the degree to which the implicit midpoint and generalized leapfrog integrators violate reversibility and volume preservation on Neal's funnel distribution. We observe that the implicit midpoint integrator exhibits better symmetry and volume preservation. {\bf The implicit midpoint is represented by the symbol $(\boldsymbol{\cdot})$ and the generalized leapfrog by the symbol $(+)$.}}
    \label{fig:neal-funnel-symmetry-volume}
\end{figure*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/figures/stochastic-volatility-fixed-point.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{images/stochastic-volatility-fixed-point.png}
    \caption{Visualization of the relative frequency of the number of fixed point iterations in the implicit midpoint and generalized leapfrog integration procedure for the stochastic volatility model.}
    \label{fig:stochastic-volatility-fixed-point}
\end{figure*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/banana-ess.tex <==
\begin{table*}[t!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrrr}
\toprule
     &      &                            &  Acc. Prob. & Time (Sec.) &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Step Size & Num. Steps & Method &          &            &            &               &              \\
\midrule
0.1 & 5 & G.L.F.(a) & $0.62 \pm 0.01$ & $400.33 \pm 6.83$ & $486.32 \pm 17.89$ & $286.28 \pm 16.09$ & $1.21 \pm 0.04$ & $0.71 \pm 0.04$ \\
& & G.L.F.(b) & $0.61 \pm 0.01$ & $145.99 \pm 2.20$ & $491.07 \pm 22.03$ & $301.90 \pm 16.21$ & $3.36 \pm 0.13$ & $2.07 \pm 0.10$ \\
& & I.M.(a) & $0.98 \pm 0.00$ & $102.37 \pm 1.13$ & $884.09 \pm 27.39$ & $620.26 \pm 30.08$ & $8.65 \pm 0.31$ & $6.07 \pm 0.32$ \\
& & I.M.(b) & $0.98 \pm 0.00$ & $95.28 \pm 2.28$ & $857.61 \pm 24.99$ & $619.91 \pm 27.09$ & $9.03 \pm 0.28$ & $6.53 \pm 0.31$ \\
& 10 & G.L.F.(a) & $0.50 \pm 0.01$ & $615.14 \pm 6.51$ & $1038.47 \pm 25.68$ & $778.80 \pm 30.92$ & $1.69 \pm 0.05$ & $1.27 \pm 0.05$ \\
& & G.L.F.(b) & $0.49 \pm 0.01$ & $231.55 \pm 2.48$ & $1027.78 \pm 25.19$ & $782.85 \pm 14.87$ & $4.44 \pm 0.12$ & $3.38 \pm 0.07$ \\
& & I.M.(a) & $0.98 \pm 0.00$ & $194.82 \pm 2.39$ & $3018.50 \pm 70.23$ & $2518.65 \pm 83.19$ & $15.51 \pm 0.39$ & $12.94 \pm 0.43$ \\
& & I.M.(b) & $0.98 \pm 0.00$ & $172.12 \pm 1.45$ & $3025.14 \pm 55.19$ & $2540.88 \pm 99.95$ & $17.58 \pm 0.34$ & $14.76 \pm 0.56$ \\
& 50 & G.L.F.(a) & $0.13 \pm 0.00$ & $2133.63 \pm 64.84$ & $192.82 \pm 24.27$ & $79.12 \pm 14.55$ & $0.09 \pm 0.01$ & $0.04 \pm 0.01$ \\
& & G.L.F.(b) & $0.14 \pm 0.00$ & $786.40 \pm 18.50$ & $247.58 \pm 28.90$ & $119.23 \pm 18.68$ & $0.31 \pm 0.03$ & $0.15 \pm 0.02$ \\
& & I.M.(a) & $0.95 \pm 0.00$ & $938.79 \pm 15.17$ & $4173.70 \pm 199.89$ & $3207.59 \pm 113.94$ & $4.47 \pm 0.25$ & $3.43 \pm 0.14$ \\
& & I.M.(b) & $0.95 \pm 0.00$ & $834.63 \pm 13.42$ & $3928.27 \pm 159.13$ & $3158.40 \pm 93.76$ & $4.73 \pm 0.24$ & $3.80 \pm 0.15$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and generalized leapfrog integrators on sampling from the banana-shaped distribution. To assess performance of the sampler, we measure the effective sample size (ESS) and present per-second timing comparisons for the mean and minimum ESS. The hypothesis that the implicit midpoint integrator should exhibit better energy conservation is captured in the acceptance probability of the Markov chain. Results are averaged over ten trials.}
    \label{tab:banana-ess}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/fitzhugh-nagumo-ess.tex <==
\begin{table*}[t!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrrr}
\toprule
     &      &                            &  Acc. Prob. & Time (Sec.) &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Step Size & Num. Steps & Method &          &            &            &               &              \\
\midrule
1.0 & 1 & G.L.F.(a) & $0.74 \pm 0.01$ & $4441.16 \pm 117.73$ & $276.39 \pm 13.48$ & $235.39 \pm 10.55$ & $0.06 \pm 0.00$ & $0.05 \pm 0.00$ \\
& & G.L.F.(b) & $0.73 \pm 0.01$ & $1343.63 \pm 76.12$ & $272.72 \pm 7.96$ & $235.52 \pm 8.99$ & $0.21 \pm 0.01$ & $0.18 \pm 0.01$ \\
& & I.M.(a) & $0.95 \pm 0.00$ & $4523.49 \pm 160.00$ & $227.01 \pm 13.47$ & $199.10 \pm 13.70$ & $0.05 \pm 0.00$ & $0.04 \pm 0.00$ \\
& & I.M.(b) & $0.95 \pm 0.00$ & $4486.29 \pm 147.33$ & $248.11 \pm 8.74$ & $225.67 \pm 9.11$ & $0.06 \pm 0.00$ & $0.05 \pm 0.00$ \\
& 2 & G.L.F.(a) & $0.74 \pm 0.01$ & $8100.90 \pm 423.17$ & $1089.36 \pm 55.17$ & $907.30 \pm 75.02$ & $0.14 \pm 0.01$ & $0.11 \pm 0.01$ \\
& & G.L.F.(b) & $0.75 \pm 0.01$ & $1912.73 \pm 48.99$ & $1109.78 \pm 71.50$ & $917.52 \pm 98.66$ & $0.58 \pm 0.04$ & $0.48 \pm 0.05$ \\
& & I.M.(a) & $0.94 \pm 0.00$ & $8704.37 \pm 250.22$ & $1387.96 \pm 40.53$ & $1212.91 \pm 42.68$ & $0.16 \pm 0.01$ & $0.14 \pm 0.01$ \\
& & I.M.(b) & $0.94 \pm 0.00$ & $8423.40 \pm 139.60$ & $1366.07 \pm 56.59$ & $1213.01 \pm 55.18$ & $0.16 \pm 0.00$ & $0.14 \pm 0.01$ \\
& 5 & G.L.F.(a) & $0.70 \pm 0.01$ & $20096.64 \pm 384.16$ & $188.59 \pm 27.78$ & $90.00 \pm 19.15$ & $0.01 \pm 0.00$ & $0.00 \pm 0.00$ \\
& & G.L.F.(b) & $0.71 \pm 0.01$ & $5138.31 \pm 300.83$ & $150.03 \pm 23.06$ & $102.32 \pm 22.10$ & $0.03 \pm 0.00$ & $0.02 \pm 0.00$ \\
& & I.M.(a) & $0.94 \pm 0.00$ & $22069.48 \pm 650.03$ & $954.94 \pm 93.17$ & $818.16 \pm 91.14$ & $0.04 \pm 0.01$ & $0.04 \pm 0.01$ \\
& & I.M.(b) & $0.94 \pm 0.00$ & $20575.78 \pm 506.21$ & $1095.88 \pm 130.14$ & $821.77 \pm 80.15$ & $0.05 \pm 0.01$ & $0.04 \pm 0.00$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and generalized leapfrog integrators on sampling from the posterior of the Fitzhugh-Nagumo model. In this example, the higher acceptance probability of the implicit midpoint integrator did not produce a performance increase for a single integration step. The implicit midpoint integrator becomes super-efficient in the two-step regime, but cannot compete with the generalized leapfrog integrator's computational advantages.}
    \label{tab:fitzhugh-nagumo-ess}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/logistic-regression-breast-cancer.tex <==
\begin{table*}[t!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrr}
\toprule
     &      &                            &  Acc. Prob. &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Step Size & Num. Steps & Method &          &            &            &               &              \\
\midrule
0.1 & 5 & G.L.F.(a) & $1.00 \pm 0.00$ & $657.70 \pm 7.91$ & $544.12 \pm 14.20$ & $5.10 \pm 0.09$ & $4.22 \pm 0.13$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $656.40 \pm 8.22$ & $530.78 \pm 14.66$ & $11.64 \pm 0.19$ & $9.42 \pm 0.31$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $644.86 \pm 5.96$ & $525.95 \pm 12.06$ & $5.18 \pm 0.05$ & $4.22 \pm 0.10$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $653.46 \pm 7.75$ & $521.33 \pm 15.77$ & $5.98 \pm 0.09$ & $4.77 \pm 0.15$ \\
& 10 & G.L.F.(a) & $1.00 \pm 0.00$ & $3011.19 \pm 22.56$ & $2763.67 \pm 35.50$ & $12.33 \pm 0.10$ & $11.32 \pm 0.17$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $3013.59 \pm 13.75$ & $2686.52 \pm 48.17$ & $29.85 \pm 0.19$ & $26.61 \pm 0.44$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $3000.27 \pm 17.29$ & $2721.65 \pm 36.14$ & $12.60 \pm 0.09$ & $11.43 \pm 0.17$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $2982.78 \pm 15.14$ & $2716.33 \pm 43.65$ & $14.42 \pm 0.16$ & $13.13 \pm 0.27$ \\
& 50 & G.L.F.(a) & $1.00 \pm 0.00$ & $5090.37 \pm 28.81$ & $4650.52 \pm 57.69$ & $4.29 \pm 0.03$ & $3.92 \pm 0.06$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $5071.69 \pm 26.96$ & $4660.23 \pm 57.15$ & $11.08 \pm 0.09$ & $10.18 \pm 0.15$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $5155.52 \pm 38.72$ & $4734.41 \pm 52.70$ & $4.48 \pm 0.03$ & $4.12 \pm 0.04$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $5190.77 \pm 22.02$ & $4739.59 \pm 64.52$ & $5.23 \pm 0.05$ & $4.78 \pm 0.09$ \\ \midrule
1.0 & 5 & G.L.F.(a) & $0.19 \pm 0.02$ & $113.18 \pm 10.39$ & $61.40 \pm 9.69$ & $0.37 \pm 0.03$ & $0.20 \pm 0.03$ \\
& & G.L.F.(b) & $0.21 \pm 0.00$ & $147.14 \pm 5.94$ & $79.51 \pm 9.49$ & $1.57 \pm 0.06$ & $0.85 \pm 0.10$ \\
& & I.M.(a) & $0.88 \pm 0.00$ & $7338.66 \pm 40.87$ & $6284.89 \pm 141.01$ & $17.05 \pm 0.15$ & $14.60 \pm 0.32$ \\
& & I.M.(b) & $0.87 \pm 0.00$ & $7355.17 \pm 56.08$ & $6418.95 \pm 173.52$ & $17.93 \pm 0.16$ & $15.65 \pm 0.42$ \\
& 10 & G.L.F.(a) & $0.14 \pm 0.00$ & $181.31 \pm 22.14$ & $87.52 \pm 19.51$ & $0.45 \pm 0.05$ & $0.21 \pm 0.05$ \\
& & G.L.F.(b) & $0.14 \pm 0.00$ & $178.90 \pm 19.79$ & $90.50 \pm 17.22$ & $1.48 \pm 0.16$ & $0.75 \pm 0.14$ \\
& & I.M.(a) & $0.86 \pm 0.00$ & $31253.10 \pm 1766.12$ & $17610.80 \pm 2459.35$ & $35.43 \pm 2.34$ & $20.10 \pm 2.93$ \\
& & I.M.(b) & $0.86 \pm 0.00$ & $29505.12 \pm 1650.54$ & $17108.46 \pm 2719.39$ & $35.27 \pm 2.06$ & $20.49 \pm 3.30$ \\
& 50 & G.L.F.(a) & $0.06 \pm 0.00$ & $71.76 \pm 9.80$ & $20.62 \pm 5.41$ & $0.10 \pm 0.01$ & $0.03 \pm 0.01$ \\
& & G.L.F.(b) & $0.06 \pm 0.01$ & $108.39 \pm 25.71$ & $44.92 \pm 16.60$ & $0.47 \pm 0.10$ & $0.19 \pm 0.07$ \\
& & I.M.(a) & $0.83 \pm 0.00$ & $10127.12 \pm 327.96$ & $4430.28 \pm 278.92$ & $2.07 \pm 0.07$ & $0.91 \pm 0.06$ \\
& & I.M.(b) & $0.83 \pm 0.00$ & $10162.12 \pm 417.45$ & $4173.36 \pm 445.85$ & $2.20 \pm 0.10$ & $0.91 \pm 0.10$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and generalized leapfrog integrators on sampling from the Bayesian logistic regression posterior on the Breast Cancer dataset. For the larger step-size, the acceptance rate of the generalized leapfrog integrator completely deteriorates whereas the implicit midpoint integrator is more robust. The implicit midpoint integrator is able to achieve super-efficient sampling for a step-size of $\epsilon=1$ and ten integration steps.}
    \label{tab:logistic-regression-breast-cancer}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/logistic-regression-diabetes.tex <==
\begin{table*}[t!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrr}
\toprule
     &      &                            &  Acc. Prob. &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Step Size & Num. Steps & Method &          &            &            &               &              \\
\midrule
0.1 & 5 & G.L.F.(a) & $1.00 \pm 0.00$ & $651.60 \pm 10.19$ & $529.61 \pm 24.09$ & $4.21 \pm 0.06$ & $3.42 \pm 0.16$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $647.30 \pm 8.08$ & $544.38 \pm 14.30$ & $10.13 \pm 0.15$ & $8.52 \pm 0.23$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $649.67 \pm 5.17$ & $531.52 \pm 18.59$ & $3.84 \pm 0.06$ & $3.14 \pm 0.11$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $647.56 \pm 10.04$ & $537.62 \pm 16.70$ & $4.41 \pm 0.08$ & $3.67 \pm 0.13$ \\
& 10 & G.L.F.(a) & $1.00 \pm 0.00$ & $2986.69 \pm 23.91$ & $2705.46 \pm 58.58$ & $10.16 \pm 0.09$ & $9.20 \pm 0.19$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $2964.67 \pm 17.29$ & $2715.30 \pm 34.13$ & $26.06 \pm 0.39$ & $23.88 \pm 0.51$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $2959.34 \pm 21.18$ & $2741.55 \pm 35.33$ & $9.18 \pm 0.10$ & $8.51 \pm 0.12$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $2963.56 \pm 17.48$ & $2710.39 \pm 58.89$ & $10.78 \pm 0.08$ & $9.86 \pm 0.21$ \\
& 50 & G.L.F.(a) & $1.00 \pm 0.00$ & $5393.71 \pm 31.87$ & $5047.21 \pm 52.74$ & $3.80 \pm 0.03$ & $3.55 \pm 0.04$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $5403.67 \pm 40.17$ & $4966.93 \pm 71.68$ & $10.53 \pm 0.09$ & $9.68 \pm 0.14$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $5445.70 \pm 35.37$ & $5069.47 \pm 87.22$ & $3.51 \pm 0.03$ & $3.27 \pm 0.06$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $5529.36 \pm 24.08$ & $5161.12 \pm 39.27$ & $4.14 \pm 0.02$ & $3.86 \pm 0.03$ \\ \midrule
1.0 & 5 & G.L.F.(a) & $0.71 \pm 0.00$ & $1507.07 \pm 28.17$ & $1051.41 \pm 56.24$ & $4.78 \pm 0.10$ & $3.34 \pm 0.18$ \\
& & G.L.F.(b) & $0.71 \pm 0.00$ & $1533.13 \pm 19.75$ & $1136.48 \pm 40.48$ & $16.78 \pm 0.17$ & $12.45 \pm 0.46$ \\
& & I.M.(a) & $0.97 \pm 0.00$ & $10484.51 \pm 46.67$ & $9934.74 \pm 60.88$ & $18.74 \pm 0.08$ & $17.76 \pm 0.12$ \\
& & I.M.(b) & $0.97 \pm 0.00$ & $10446.28 \pm 28.06$ & $9870.19 \pm 65.18$ & $19.71 \pm 0.13$ & $18.62 \pm 0.17$ \\
& 10 & G.L.F.(a) & $0.60 \pm 0.00$ & $4878.12 \pm 107.69$ & $2912.57 \pm 257.17$ & $7.89 \pm 0.18$ & $4.71 \pm 0.42$ \\
& & G.L.F.(b) & $0.60 \pm 0.00$ & $5088.12 \pm 42.63$ & $3495.29 \pm 126.45$ & $30.17 \pm 0.28$ & $20.71 \pm 0.73$ \\
& & I.M.(a) & $0.97 \pm 0.00$ & $40000.00 \pm 0.00$ & $40000.00 \pm 0.00$ & $36.32 \pm 0.13$ & $36.32 \pm 0.13$ \\
& & I.M.(b) & $0.96 \pm 0.00$ & $40000.00 \pm 0.00$ & $40000.00 \pm 0.00$ & $38.39 \pm 0.08$ & $38.39 \pm 0.08$ \\
& 50 & G.L.F.(a) & $0.64 \pm 0.00$ & $6454.94 \pm 278.39$ & $4318.50 \pm 306.57$ & $2.32 \pm 0.10$ & $1.55 \pm 0.11$ \\
& & G.L.F.(b) & $0.64 \pm 0.00$ & $6357.53 \pm 179.10$ & $4245.83 \pm 213.30$ & $8.75 \pm 0.24$ & $5.84 \pm 0.29$ \\
& & I.M.(a) & $0.97 \pm 0.00$ & $37135.14 \pm 210.27$ & $20941.08 \pm 409.25$ & $6.77 \pm 0.04$ & $3.82 \pm 0.07$ \\
& & I.M.(b) & $0.97 \pm 0.00$ & $37049.46 \pm 189.78$ & $20932.03 \pm 441.83$ & $7.02 \pm 0.09$ & $3.97 \pm 0.10$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and generalized leapfrog integrators on sampling from the Bayesian logistic regression posterior on the Diabetes dataset.}
    \label{tab:logistic-regression-diabetes}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/logistic-regression-heart.tex <==
\begin{table*}[t!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrr}
\toprule
     &      &                            &  Acc. Prob. &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Step Size & Num. Steps & Method &          &            &            &               &              \\
\midrule
0.1 & 5 & G.L.F.(a) & $1.00 \pm 0.00$ & $653.84 \pm 8.93$ & $541.18 \pm 16.32$ & $3.86 \pm 0.05$ & $3.19 \pm 0.10$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $656.59 \pm 6.98$ & $533.13 \pm 11.07$ & $9.55 \pm 0.15$ & $7.75 \pm 0.18$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $668.14 \pm 4.07$ & $564.02 \pm 8.36$ & $4.23 \pm 0.04$ & $3.57 \pm 0.05$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $664.05 \pm 6.83$ & $517.75 \pm 15.55$ & $4.78 \pm 0.08$ & $3.73 \pm 0.14$ \\
& 10 & G.L.F.(a) & $0.99 \pm 0.00$ & $3019.18 \pm 16.31$ & $2659.45 \pm 40.27$ & $9.13 \pm 0.17$ & $8.05 \pm 0.21$ \\
& & G.L.F.(b) & $0.99 \pm 0.00$ & $3021.32 \pm 18.34$ & $2686.55 \pm 45.81$ & $24.54 \pm 0.28$ & $21.83 \pm 0.47$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $3019.84 \pm 16.66$ & $2728.01 \pm 27.65$ & $9.82 \pm 0.07$ & $8.86 \pm 0.06$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $3029.96 \pm 13.91$ & $2683.39 \pm 43.94$ & $11.42 \pm 0.10$ & $10.12 \pm 0.19$ \\
& 50 & G.L.F.(a) & $0.99 \pm 0.00$ & $4934.18 \pm 14.56$ & $4500.43 \pm 42.68$ & $3.14 \pm 0.02$ & $2.86 \pm 0.03$ \\
& & G.L.F.(b) & $0.99 \pm 0.00$ & $4952.56 \pm 14.79$ & $4431.26 \pm 54.96$ & $8.84 \pm 0.07$ & $7.91 \pm 0.11$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $5107.34 \pm 20.29$ & $4626.57 \pm 72.19$ & $3.44 \pm 0.01$ & $3.12 \pm 0.05$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $5089.77 \pm 21.30$ & $4642.54 \pm 54.89$ & $4.02 \pm 0.02$ & $3.67 \pm 0.04$ \\ \midrule
1.0 & 5 & G.L.F.(a) & $0.05 \pm 0.00$ & $25.97 \pm 3.33$ & $7.21 \pm 1.36$ & $0.08 \pm 0.01$ & $0.02 \pm 0.00$ \\
& & G.L.F.(b) & $0.05 \pm 0.00$ & $29.48 \pm 2.90$ & $9.96 \pm 2.03$ & $0.37 \pm 0.04$ & $0.13 \pm 0.03$ \\
& & I.M.(a) & $0.70 \pm 0.00$ & $4335.06 \pm 63.32$ & $3250.56 \pm 138.84$ & $6.53 \pm 0.12$ & $4.90 \pm 0.21$ \\
& & I.M.(b) & $0.70 \pm 0.00$ & $4352.91 \pm 83.82$ & $3300.84 \pm 186.04$ & $6.51 \pm 0.19$ & $4.95 \pm 0.31$ \\
& 10 & G.L.F.(a) & $0.03 \pm 0.00$ & $44.35 \pm 4.24$ & $12.20 \pm 1.90$ & $0.12 \pm 0.01$ & $0.03 \pm 0.00$ \\
& & G.L.F.(b) & $0.02 \pm 0.00$ & $44.07 \pm 8.26$ & $10.00 \pm 1.91$ & $0.51 \pm 0.11$ & $0.11 \pm 0.02$ \\
& & I.M.(a) & $0.66 \pm 0.00$ & $9217.63 \pm 305.79$ & $5320.85 \pm 661.55$ & $5.45 \pm 0.21$ & $3.16 \pm 0.41$ \\
& & I.M.(b) & $0.66 \pm 0.00$ & $9752.37 \pm 315.58$ & $5172.40 \pm 382.12$ & $5.72 \pm 0.20$ & $3.05 \pm 0.24$ \\
& 50 & G.L.F.(a) & $0.01 \pm 0.00$ & $19.19 \pm 3.58$ & $4.62 \pm 0.55$ & $0.05 \pm 0.02$ & $0.01 \pm 0.00$ \\
& & G.L.F.(b) & $0.01 \pm 0.00$ & $24.34 \pm 7.90$ & $5.81 \pm 1.41$ & $0.21 \pm 0.07$ & $0.05 \pm 0.01$ \\
& & I.M.(a) & $0.58 \pm 0.00$ & $2818.14 \pm 244.09$ & $1287.74 \pm 212.68$ & $0.22 \pm 0.02$ & $0.10 \pm 0.02$ \\
& & I.M.(b) & $0.58 \pm 0.01$ & $3028.35 \pm 370.09$ & $1445.54 \pm 329.95$ & $0.25 \pm 0.03$ & $0.12 \pm 0.03$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and generalized leapfrog integrators on sampling from the Bayesian logistic regression posterior on the heart disease dataset.}
    \label{tab:logistic-regression-heart}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/neal-funnel-ess.tex <==
\begin{table*}[t!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrrr}
\toprule
     &      &                            &  Acc. Prob. & Time (Sec.) &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Num. Steps & Step Size & Method &          &            &            &               &              \\
\midrule
20 & 0.1 & G.L.F.(a) & $0.99 \pm 0.00$ & $1317.57 \pm 16.89$ & $15614.52 \pm 177.89$ & $340.56 \pm 17.41$ & $11.86 \pm 0.16$ & $0.26 \pm 0.01$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $1315.24 \pm 57.79$ & $16199.00 \pm 157.60$ & $383.48 \pm 22.16$ & $12.47 \pm 0.44$ & $0.30 \pm 0.02$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $1147.45 \pm 64.92$ & $15697.78 \pm 148.81$ & $392.22 \pm 23.11$ & $14.02 \pm 0.74$ & $0.35 \pm 0.03$ \\
& 0.2 & G.L.F.(a) & $0.96 \pm 0.00$ & $1933.64 \pm 97.74$ & $29457.72 \pm 353.68$ & $1511.75 \pm 28.61$ & $15.55 \pm 0.79$ & $0.79 \pm 0.03$ \\
& & I.M.(a) & $0.99 \pm 0.00$ & $1669.69 \pm 78.93$ & $32055.29 \pm 257.52$ & $1588.73 \pm 54.01$ & $19.52 \pm 0.86$ & $0.96 \pm 0.05$ \\
& & I.M.(b) & $0.99 \pm 0.00$ & $1441.81 \pm 61.06$ & $31585.28 \pm 197.07$ & $1558.54 \pm 36.83$ & $22.17 \pm 0.79$ & $1.10 \pm 0.05$ \\
& 0.5 & G.L.F.(a) & $0.36 \pm 0.00$ & $2389.27 \pm 49.42$ & $2144.93 \pm 103.34$ & $1771.92 \pm 140.71$ & $0.90 \pm 0.05$ & $0.74 \pm 0.06$ \\
& & I.M.(a) & $0.85 \pm 0.00$ & $2981.80 \pm 71.09$ & $10984.29 \pm 123.63$ & $10147.33 \pm 121.32$ & $3.70 \pm 0.09$ & $3.42 \pm 0.07$ \\
& & I.M.(b) & $0.85 \pm 0.00$ & $2728.61 \pm 82.50$ & $10563.94 \pm 210.16$ & $9711.29 \pm 264.30$ & $3.90 \pm 0.13$ & $3.58 \pm 0.13$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and the naive generalized leapfrog integrators on sampling from Neal's funnel distribution. We see that the implicit midpoint integrator is able to take large steps and produce an effective sample size that outperforms the generalized leapfrog integrator even in the time-normalized performance.}
    \label{tab:neal-funnel-ess}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/randomized-step-banana-ess.tex <==
\begin{table*}[b!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrrr}
\toprule
     &      &                            &  Acc. Prob. & Time (Sec.) &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Step Size & Max. Steps & Method &          &            &            &               &              \\
\midrule
0.1 & 5 & G.L.F.(a) & $0.66 \pm 0.01$ & $298.11 \pm 4.99$ & $240.50 \pm 13.01$ & $140.54 \pm 10.54$ & $0.81 \pm 0.04$ & $0.47 \pm 0.03$ \\
& & G.L.F.(b) & $0.66 \pm 0.01$ & $103.90 \pm 1.64$ & $246.99 \pm 10.57$ & $149.70 \pm 8.26$ & $2.37 \pm 0.08$ & $1.44 \pm 0.07$ \\
& & I.M.(a) & $0.99 \pm 0.00$ & $65.48 \pm 0.97$ & $372.91 \pm 20.52$ & $276.00 \pm 18.41$ & $5.69 \pm 0.28$ & $4.20 \pm 0.24$ \\
& & I.M.(b) & $0.99 \pm 0.00$ & $59.90 \pm 0.98$ & $375.99 \pm 23.34$ & $268.26 \pm 15.80$ & $6.32 \pm 0.45$ & $4.51 \pm 0.30$ \\
& 10 & G.L.F.(a) & $0.60 \pm 0.01$ & $420.38 \pm 8.68$ & $541.71 \pm 13.63$ & $373.56 \pm 16.10$ & $1.29 \pm 0.05$ & $0.89 \pm 0.04$ \\
& & G.L.F.(b) & $0.59 \pm 0.00$ & $153.94 \pm 3.34$ & $560.73 \pm 12.99$ & $370.12 \pm 13.86$ & $3.66 \pm 0.12$ & $2.41 \pm 0.11$ \\
& & I.M.(a) & $0.98 \pm 0.00$ & $111.84 \pm 1.64$ & $1205.85 \pm 38.74$ & $945.21 \pm 35.13$ & $10.80 \pm 0.37$ & $8.47 \pm 0.34$ \\
& & I.M.(b) & $0.98 \pm 0.00$ & $100.24 \pm 1.79$ & $1212.95 \pm 41.28$ & $948.95 \pm 47.69$ & $12.12 \pm 0.42$ & $9.47 \pm 0.46$ \\
& 50 & G.L.F.(a) & $0.31 \pm 0.00$ & $1158.96 \pm 13.35$ & $744.51 \pm 34.97$ & $603.15 \pm 17.87$ & $0.64 \pm 0.03$ & $0.52 \pm 0.02$ \\
& & G.L.F.(b) & $0.31 \pm 0.01$ & $451.75 \pm 4.30$ & $754.07 \pm 37.32$ & $602.83 \pm 42.83$ & $1.67 \pm 0.09$ & $1.34 \pm 0.10$ \\
& & I.M.(a) & $0.97 \pm 0.00$ & $473.24 \pm 4.62$ & $6306.89 \pm 136.15$ & $2568.88 \pm 34.70$ & $13.33 \pm 0.28$ & $5.43 \pm 0.07$ \\
& & I.M.(b) & $0.97 \pm 0.00$ & $419.67 \pm 3.65$ & $6345.83 \pm 165.83$ & $2597.81 \pm 50.49$ & $15.14 \pm 0.46$ & $6.20 \pm 0.14$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and generalized leapfrog integrators on sampling from the banana-shaped distribution when a randomized number of steps is used.}
    \label{tab:randomized-step-banana-ess}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/randomized-step-fitzhugh-nagumo.tex <==
\begin{table*}[t!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrrr}
\toprule
     &      &                            &  Acc. Prob. & Time (Sec.) &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Step Size & Num. Steps & Method &          &            &            &               &              \\
\midrule
1.0 & 1 & G.L.F.(a) & $0.75 \pm 0.01$ & $4084.16 \pm 138.81$ & $289.87 \pm 12.89$ & $251.36 \pm 12.33$ & $0.07 \pm 0.01$ & $0.06 \pm 0.00$ \\
& & G.L.F.(b) & $0.74 \pm 0.01$ & $1193.08 \pm 61.74$ & $301.44 \pm 16.67$ & $262.36 \pm 15.38$ & $0.26 \pm 0.02$ & $0.23 \pm 0.02$ \\
& & I.M.(a) & $0.95 \pm 0.00$ & $4353.40 \pm 104.50$ & $237.73 \pm 8.67$ & $219.04 \pm 11.18$ & $0.05 \pm 0.00$ & $0.05 \pm 0.00$ \\
& & I.M.(b) & $0.95 \pm 0.00$ & $4539.73 \pm 132.69$ & $228.33 \pm 8.69$ & $191.36 \pm 9.91$ & $0.05 \pm 0.00$ & $0.04 \pm 0.00$ \\
& 2 & G.L.F.(a) & $0.75 \pm 0.01$ & $6265.35 \pm 187.70$ & $620.36 \pm 17.86$ & $553.05 \pm 20.54$ & $0.10 \pm 0.00$ & $0.09 \pm 0.00$ \\
& & G.L.F.(b) & $0.74 \pm 0.01$ & $1743.26 \pm 61.19$ & $592.04 \pm 12.90$ & $518.75 \pm 16.25$ & $0.35 \pm 0.02$ & $0.30 \pm 0.02$ \\
& & I.M.(a) & $0.94 \pm 0.00$ & $7051.31 \pm 190.41$ & $612.50 \pm 23.74$ & $543.62 \pm 27.06$ & $0.09 \pm 0.00$ & $0.08 \pm 0.00$ \\
& & I.M.(b) & $0.94 \pm 0.00$ & $6549.13 \pm 146.01$ & $626.26 \pm 16.04$ & $566.83 \pm 19.62$ & $0.10 \pm 0.00$ & $0.09 \pm 0.00$ \\
& 5 & G.L.F.(a) & $0.74 \pm 0.01$ & $12447.27 \pm 560.25$ & $726.90 \pm 53.55$ & $629.11 \pm 64.83$ & $0.06 \pm 0.01$ & $0.05 \pm 0.01$ \\
& & G.L.F.(b) & $0.74 \pm 0.01$ & $2974.54 \pm 90.05$ & $756.32 \pm 49.99$ & $637.53 \pm 61.54$ & $0.26 \pm 0.02$ & $0.22 \pm 0.02$ \\
& & I.M.(a) & $0.94 \pm 0.00$ & $13331.24 \pm 263.47$ & $1320.95 \pm 77.86$ & $1106.66 \pm 81.97$ & $0.10 \pm 0.01$ & $0.08 \pm 0.01$ \\
& & I.M.(b) & $0.93 \pm 0.00$ & $12501.60 \pm 457.80$ & $1441.09 \pm 54.15$ & $1229.29 \pm 63.45$ & $0.12 \pm 0.01$ & $0.10 \pm 0.01$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and generalized leapfrog integrators on sampling from the posterior of the Fitzhugh-Nagumo model when a randomized number of integration steps are used.}
    \label{tab:randomized-step-fitzhugh-nagumo-ess}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/randomized-step-logistic-regression-breast-cancer.tex <==
\begin{table*}[t!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrr}
\toprule
     &      &                            &  Acc. Prob. &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Step Size & Max. Steps & Method &          &            &            &               &              \\
\midrule
0.1 & 5 & G.L.F.(a) & $1.00 \pm 0.00$ & $286.35 \pm 4.21$ & $208.68 \pm 9.49$ & $3.50 \pm 0.06$ & $2.55 \pm 0.12$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $283.91 \pm 5.17$ & $212.44 \pm 8.27$ & $7.18 \pm 0.16$ & $5.39 \pm 0.25$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $283.77 \pm 4.26$ & $222.26 \pm 9.88$ & $3.58 \pm 0.06$ & $2.80 \pm 0.13$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $286.73 \pm 4.68$ & $221.40 \pm 12.74$ & $4.15 \pm 0.07$ & $3.20 \pm 0.19$ \\
& 10 & G.L.F.(a) & $1.00 \pm 0.00$ & $1010.60 \pm 11.69$ & $893.84 \pm 20.10$ & $7.22 \pm 0.10$ & $6.39 \pm 0.16$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $1002.32 \pm 15.93$ & $873.10 \pm 21.47$ & $16.45 \pm 0.27$ & $14.33 \pm 0.35$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $1005.16 \pm 12.23$ & $871.72 \pm 15.41$ & $7.50 \pm 0.07$ & $6.50 \pm 0.10$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $1021.59 \pm 8.10$ & $887.65 \pm 27.54$ & $8.48 \pm 0.19$ & $7.37 \pm 0.28$ \\
& 50 & G.L.F.(a) & $1.00 \pm 0.00$ & $14410.27 \pm 147.75$ & $13303.56 \pm 189.57$ & $23.89 \pm 0.19$ & $22.05 \pm 0.26$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $14411.21 \pm 90.58$ & $13450.61 \pm 91.65$ & $60.17 \pm 0.33$ & $56.16 \pm 0.29$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $14548.15 \pm 121.78$ & $13483.46 \pm 126.40$ & $24.79 \pm 0.19$ & $22.98 \pm 0.22$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $14519.88 \pm 118.88$ & $13317.24 \pm 127.50$ & $28.52 \pm 0.25$ & $26.16 \pm 0.29$ \\ \midrule
1.0 & 5 & G.L.F.(a) & $0.23 \pm 0.00$ & $904.47 \pm 54.85$ & $542.07 \pm 69.66$ & $4.10 \pm 0.23$ & $2.45 \pm 0.31$ \\
& & G.L.F.(b) & $0.23 \pm 0.00$ & $900.64 \pm 23.10$ & $596.22 \pm 40.82$ & $12.66 \pm 0.37$ & $8.37 \pm 0.56$ \\
& & I.M.(a) & $0.89 \pm 0.00$ & $12294.41 \pm 127.45$ & $10991.38 \pm 217.01$ & $47.59 \pm 0.55$ & $42.55 \pm 0.87$ \\
& & I.M.(b) & $0.89 \pm 0.00$ & $12506.83 \pm 182.42$ & $11280.48 \pm 316.77$ & $50.82 \pm 0.68$ & $45.82 \pm 1.21$ \\
& 10 & G.L.F.(a) & $0.19 \pm 0.00$ & $663.43 \pm 35.45$ & $417.15 \pm 38.40$ & $2.25 \pm 0.11$ & $1.41 \pm 0.12$ \\
& & G.L.F.(b) & $0.19 \pm 0.00$ & $568.08 \pm 31.76$ & $333.88 \pm 39.54$ & $6.32 \pm 0.31$ & $3.69 \pm 0.40$ \\
& & I.M.(a) & $0.87 \pm 0.00$ & $8312.69 \pm 53.82$ & $7449.40 \pm 86.13$ & $17.09 \pm 0.23$ & $15.31 \pm 0.23$ \\
& & I.M.(b) & $0.88 \pm 0.00$ & $8306.90 \pm 46.45$ & $7407.88 \pm 136.86$ & $18.24 \pm 0.19$ & $16.27 \pm 0.36$ \\
& 50 & G.L.F.(a) & $0.10 \pm 0.00$ & $218.25 \pm 33.24$ & $119.54 \pm 22.69$ & $0.41 \pm 0.06$ & $0.22 \pm 0.04$ \\
& & G.L.F.(b) & $0.10 \pm 0.00$ & $199.52 \pm 25.14$ & $110.61 \pm 21.56$ & $1.26 \pm 0.15$ & $0.70 \pm 0.13$ \\
& & I.M.(a) & $0.85 \pm 0.00$ & $6422.28 \pm 65.69$ & $5107.53 \pm 212.97$ & $2.63 \pm 0.04$ & $2.09 \pm 0.08$ \\
& & I.M.(b) & $0.85 \pm 0.00$ & $6693.87 \pm 72.47$ & $5565.30 \pm 272.50$ & $2.90 \pm 0.05$ & $2.41 \pm 0.13$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and generalized leapfrog integrators on sampling from the Bayesian logistic regression posterior on the Breast Cancer dataset when using a randomized number of integration steps.}
    \label{tab:randomized-step-logistic-regression-breast-cancer}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/randomized-step-logistic-regression-diabetes.tex <==
\begin{table*}[t!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrr}
\toprule
     &      &                            &  Acc. Prob. &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Step Size & Max. Steps & Method &          &            &            &               &              \\
\midrule
0.1 & 5 & G.L.F.(a) & $1.00 \pm 0.00$ & $286.98 \pm 4.54$ & $234.68 \pm 7.46$ & $2.97 \pm 0.05$ & $2.43 \pm 0.07$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $280.75 \pm 3.93$ & $214.84 \pm 8.31$ & $6.39 \pm 0.09$ & $4.89 \pm 0.19$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $285.13 \pm 6.19$ & $227.96 \pm 13.22$ & $2.73 \pm 0.07$ & $2.18 \pm 0.13$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $273.54 \pm 6.51$ & $217.14 \pm 11.43$ & $2.99 \pm 0.07$ & $2.37 \pm 0.12$ \\
& 10 & G.L.F.(a) & $1.00 \pm 0.00$ & $1015.63 \pm 14.83$ & $877.03 \pm 31.16$ & $6.05 \pm 0.09$ & $5.23 \pm 0.19$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $1009.53 \pm 9.46$ & $862.28 \pm 17.84$ & $14.88 \pm 0.13$ & $12.72 \pm 0.31$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $987.06 \pm 10.31$ & $832.63 \pm 24.35$ & $5.44 \pm 0.07$ & $4.59 \pm 0.13$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $1010.27 \pm 9.23$ & $867.30 \pm 19.17$ & $6.38 \pm 0.11$ & $5.47 \pm 0.10$ \\
& 50 & G.L.F.(a) & $1.00 \pm 0.00$ & $14735.31 \pm 75.07$ & $13759.10 \pm 141.77$ & $20.13 \pm 0.17$ & $18.80 \pm 0.26$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $14774.00 \pm 99.12$ & $13680.31 \pm 124.54$ & $54.81 \pm 0.38$ & $50.75 \pm 0.49$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $14748.16 \pm 100.96$ & $13445.33 \pm 111.76$ & $18.49 \pm 0.13$ & $16.85 \pm 0.14$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $14721.71 \pm 120.84$ & $13834.19 \pm 162.68$ & $21.64 \pm 0.16$ & $20.34 \pm 0.26$ \\ \midrule
1.0 & 5 & G.L.F.(a) & $0.68 \pm 0.00$ & $7161.52 \pm 72.09$ & $6678.78 \pm 98.85$ & $37.13 \pm 0.33$ & $34.63 \pm 0.48$ \\
& & G.L.F.(b) & $0.68 \pm 0.00$ & $7132.61 \pm 58.58$ & $6617.77 \pm 98.49$ & $118.67 \pm 1.61$ & $110.15 \pm 2.30$ \\
& & I.M.(a) & $0.97 \pm 0.00$ & $16750.80 \pm 134.04$ & $15466.43 \pm 76.75$ & $49.44 \pm 0.42$ & $45.65 \pm 0.26$ \\
& & I.M.(b) & $0.97 \pm 0.00$ & $16635.79 \pm 131.54$ & $15402.22 \pm 176.98$ & $51.11 \pm 0.39$ & $47.31 \pm 0.44$ \\
& 10 & G.L.F.(a) & $0.68 \pm 0.00$ & $6498.21 \pm 53.62$ & $5885.25 \pm 55.32$ & $18.86 \pm 0.19$ & $17.08 \pm 0.20$ \\
& & G.L.F.(b) & $0.68 \pm 0.00$ & $6655.24 \pm 61.17$ & $6222.74 \pm 75.56$ & $67.37 \pm 0.79$ & $62.99 \pm 0.91$ \\
& & I.M.(a) & $0.97 \pm 0.00$ & $10858.03 \pm 109.54$ & $10245.67 \pm 118.98$ & $17.69 \pm 0.18$ & $16.70 \pm 0.20$ \\
& & I.M.(b) & $0.97 \pm 0.00$ & $10672.12 \pm 108.02$ & $10006.57 \pm 128.94$ & $18.54 \pm 0.20$ & $17.38 \pm 0.24$ \\
& 50 & G.L.F.(a) & $0.66 \pm 0.00$ & $4999.26 \pm 50.94$ & $4518.13 \pm 54.31$ & $3.41 \pm 0.04$ & $3.08 \pm 0.04$ \\
& & G.L.F.(b) & $0.66 \pm 0.00$ & $5098.68 \pm 72.88$ & $4601.08 \pm 121.45$ & $13.05 \pm 0.27$ & $11.78 \pm 0.36$ \\
& & I.M.(a) & $0.97 \pm 0.00$ & $9176.25 \pm 69.76$ & $8681.47 \pm 129.00$ & $3.27 \pm 0.03$ & $3.10 \pm 0.05$ \\
& & I.M.(b) & $0.97 \pm 0.00$ & $9176.41 \pm 58.95$ & $8657.74 \pm 87.61$ & $3.44 \pm 0.03$ & $3.24 \pm 0.03$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and generalized leapfrog integrators on sampling from the Bayesian logistic regression posterior on the Diabetes dataset when using a randomized number of steps.}
    \label{tab:randomized-step-logistic-regression-diabetes}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/randomized-step-logistic-regression-heart.tex <==
\begin{table*}[t!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrr}
\toprule
     &      &                            &  Acc. Prob. &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Step Size & Max. Steps & Method &          &            &            &               &              \\
\midrule
0.1 & 5 & G.L.F.(a) & $1.00 \pm 0.00$ & $288.33 \pm 4.45$ & $213.23 \pm 12.18$ & $2.74 \pm 0.05$ & $2.03 \pm 0.12$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $285.05 \pm 2.89$ & $208.93 \pm 12.85$ & $6.13 \pm 0.05$ & $4.49 \pm 0.28$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $284.53 \pm 2.43$ & $200.77 \pm 9.67$ & $2.86 \pm 0.02$ & $2.02 \pm 0.10$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $282.89 \pm 4.35$ & $209.47 \pm 7.53$ & $3.26 \pm 0.05$ & $2.41 \pm 0.08$ \\
& 10 & G.L.F.(a) & $1.00 \pm 0.00$ & $1026.88 \pm 6.25$ & $877.98 \pm 13.29$ & $5.50 \pm 0.08$ & $4.70 \pm 0.08$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $1010.32 \pm 7.44$ & $840.99 \pm 18.85$ & $13.45 \pm 0.24$ & $11.20 \pm 0.33$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $1023.10 \pm 9.64$ & $857.23 \pm 17.40$ & $5.89 \pm 0.05$ & $4.94 \pm 0.09$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $1026.88 \pm 11.64$ & $865.57 \pm 27.24$ & $6.75 \pm 0.10$ & $5.70 \pm 0.21$ \\
& 50 & G.L.F.(a) & $0.99 \pm 0.00$ & $14285.39 \pm 94.94$ & $13034.74 \pm 212.10$ & $17.93 \pm 0.16$ & $16.36 \pm 0.28$ \\
& & G.L.F.(b) & $1.00 \pm 0.00$ & $14327.81 \pm 86.32$ & $13322.33 \pm 153.96$ & $49.54 \pm 0.37$ & $46.07 \pm 0.61$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $14465.89 \pm 123.72$ & $13374.24 \pm 126.08$ & $19.04 \pm 0.22$ & $17.60 \pm 0.21$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $14527.88 \pm 110.84$ & $13225.19 \pm 143.07$ & $22.29 \pm 0.16$ & $20.29 \pm 0.18$ \\ \midrule
1.0 & 5 & G.L.F.(a) & $0.09 \pm 0.00$ & $348.13 \pm 17.73$ & $221.83 \pm 20.56$ & $1.35 \pm 0.08$ & $0.86 \pm 0.08$ \\
& & G.L.F.(b) & $0.09 \pm 0.00$ & $302.71 \pm 17.13$ & $194.10 \pm 18.07$ & $4.44 \pm 0.25$ & $2.84 \pm 0.25$ \\
& & I.M.(a) & $0.76 \pm 0.00$ & $8260.70 \pm 56.57$ & $6971.22 \pm 181.18$ & $21.65 \pm 0.37$ & $18.28 \pm 0.62$ \\
& & I.M.(b) & $0.76 \pm 0.00$ & $8376.43 \pm 83.15$ & $6986.00 \pm 196.62$ & $22.27 \pm 0.33$ & $18.59 \pm 0.61$ \\
& 10 & G.L.F.(a) & $0.06 \pm 0.00$ & $201.29 \pm 13.39$ & $121.49 \pm 12.69$ & $0.69 \pm 0.04$ & $0.42 \pm 0.04$ \\
& & G.L.F.(b) & $0.06 \pm 0.00$ & $212.65 \pm 19.55$ & $107.86 \pm 17.94$ & $2.68 \pm 0.24$ & $1.37 \pm 0.23$ \\
& & I.M.(a) & $0.72 \pm 0.00$ & $5371.69 \pm 83.35$ & $4242.38 \pm 174.21$ & $6.51 \pm 0.12$ & $5.15 \pm 0.23$ \\
& & I.M.(b) & $0.71 \pm 0.00$ & $5464.59 \pm 73.10$ & $4472.08 \pm 119.62$ & $6.82 \pm 0.10$ & $5.58 \pm 0.16$ \\
& 50 & G.L.F.(a) & $0.02 \pm 0.00$ & $54.25 \pm 4.75$ & $16.96 \pm 3.01$ & $0.15 \pm 0.01$ & $0.05 \pm 0.01$ \\
& & G.L.F.(b) & $0.02 \pm 0.00$ & $63.55 \pm 6.00$ & $21.88 \pm 5.09$ & $0.65 \pm 0.06$ & $0.22 \pm 0.05$ \\
& & I.M.(a) & $0.64 \pm 0.00$ & $3384.35 \pm 162.98$ & $2354.23 \pm 228.25$ & $0.57 \pm 0.03$ & $0.40 \pm 0.04$ \\
& & I.M.(b) & $0.63 \pm 0.00$ & $3381.84 \pm 58.00$ & $2217.38 \pm 190.97$ & $0.59 \pm 0.01$ & $0.39 \pm 0.03$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and generalized leapfrog integrators on sampling from the Bayesian logistic regression posterior on the heart disease dataset when using a randomized number of steps.}
    \label{tab:randomized-step-logistic-regression-heart}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/randomized-step-neal-funnel-ess.tex <==
\begin{table*}[b!]
    \centering
    \scriptsize
    \begin{tabular}{lll|rrrrrr}
\toprule
     &      &                            &  Acc. Prob. & Time (Sec.) &   Mean ESS &    Min. ESS &  Mean ESS / Sec. &  Min. ESS / Sec. \\
Max. Steps & Step Size & Method &          &            &            &               &              \\
\midrule
20 & 0.1 & G.L.F.(a) & $0.99 \pm 0.00$ & $786.17 \pm 62.99$ & $3535.77 \pm 45.31$ & $120.34 \pm 15.07$ & $4.69 \pm 0.31$ & $0.16 \pm 0.02$ \\
& & I.M.(a) & $1.00 \pm 0.00$ & $655.70 \pm 33.04$ & $3538.75 \pm 28.40$ & $132.25 \pm 12.73$ & $5.48 \pm 0.21$ & $0.21 \pm 0.02$ \\
& & I.M.(b) & $1.00 \pm 0.00$ & $579.39 \pm 40.26$ & $3545.94 \pm 32.44$ & $133.26 \pm 10.57$ & $6.29 \pm 0.31$ & $0.23 \pm 0.02$ \\
& 0.2 & G.L.F.(a) & $0.96 \pm 0.00$ & $968.70 \pm 58.97$ & $11305.65 \pm 109.81$ & $525.33 \pm 15.22$ & $11.96 \pm 0.59$ & $0.56 \pm 0.04$ \\
& & I.M.(a) & $0.99 \pm 0.00$ & $818.02 \pm 32.74$ & $11809.38 \pm 128.38$ & $502.90 \pm 33.26$ & $14.59 \pm 0.51$ & $0.63 \pm 0.05$ \\
& & I.M.(b) & $0.99 \pm 0.00$ & $728.94 \pm 21.80$ & $11959.25 \pm 115.00$ & $522.38 \pm 22.78$ & $16.52 \pm 0.51$ & $0.72 \pm 0.04$ \\
& 0.5 & G.L.F.(a) & $0.43 \pm 0.01$ & $1420.67 \pm 49.91$ & $1857.57 \pm 172.54$ & $754.50 \pm 85.59$ & $1.30 \pm 0.11$ & $0.53 \pm 0.06$ \\
& & I.M.(a) & $0.89 \pm 0.00$ & $1596.95 \pm 48.55$ & $8468.24 \pm 54.32$ & $3018.45 \pm 93.75$ & $5.34 \pm 0.15$ & $1.91 \pm 0.11$ \\
& & I.M.(b) & $0.89 \pm 0.00$ & $1458.31 \pm 53.48$ & $8422.27 \pm 57.72$ & $3034.97 \pm 81.87$ & $5.83 \pm 0.19$ & $2.10 \pm 0.09$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint and the naive generalized leapfrog integrators on sampling from Neal's funnel distribution when using a randomized number of integration steps.}
    \label{tab:randomized-step-neal-funnel-ess}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/randomized-step-stochastic-volatility-symmetry-volume-preservation.tex <==
\begin{table*}[t!]
    \centering
    \tiny
    \begin{tabular}{l|rrrrrr|rr|rr}
\toprule
       &&&&&&& \multicolumn{2}{c}{Volume Preservation} & \multicolumn{2}{c}{Symmetry} \\
    Method   & Acc. Prob. & Time (Sec.) &   Mean ESS &    Min. ESS &  \begin{tabular}[c]{@{}l@{}}Mean ESS \\ (Sec.)\end{tabular} &  \begin{tabular}[c]{@{}l@{}}Min. ESS \\ (Sec.)\end{tabular} & Median &    $90^\mathrm{th}$-Per. &  Median &    $90^\mathrm{th}$-Per. \\
\midrule
G.L.F.(a) & $0.85 \pm 0.0$ & $2367.93 \pm 16.1$ & $335.80 \pm 15.3$ & $132.96 \pm 3.9$ & $0.14 \pm 0.0$ & $0.06 \pm 0.0$ & $6.8\mathrm{e-}07$ & $2.9\mathrm{e-}06$ & $4.9\mathrm{e-}06$ & $2.4\mathrm{e-}05$ \\
G.L.F.(b) & $0.85 \pm 0.0$ & $2196.52 \pm 8.5$ & $331.84 \pm 12.1$ & $139.30 \pm 3.7$ & $0.15 \pm 0.0$ & $0.06 \pm 0.0$ & $7.1\mathrm{e-}07$ & $2.9\mathrm{e-}06$ & $4.8\mathrm{e-}06$ & $2.7\mathrm{e-}05$ \\
I.M.(a) & $0.86 \pm 0.0$ & $2434.74 \pm 7.9$ & $316.98 \pm 15.4$ & $131.79 \pm 3.4$ & $0.13 \pm 0.0$ & $0.05 \pm 0.0$ & $8.7\mathrm{e-}08$ & $2.3\mathrm{e-}07$ & $1.3\mathrm{e-}06$ & $2.4\mathrm{e-}06$ \\
I.M.(b) & $0.87 \pm 0.0$ & $2399.22 \pm 6.4$ & $342.11 \pm 14.0$ & $133.76 \pm 3.7$ & $0.14 \pm 0.0$ & $0.06 \pm 0.0$ & $1.7\mathrm{e-}07$ & $4.4\mathrm{e-}07$ & $2.8\mathrm{e-}06$ & $4.7\mathrm{e-}06$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint generalized leapfrog integrators on the stochastic volatility model when using a randomized number of integration steps.}
    \label{tab:randomized-step-stochastic-volatility-symmetry-volume-preservation}
\end{table*}

==> Evaluating the Implicit Midpoint Integrator for Riemannian Manifold Hamiltonian Manifold Monte Carlo/tables/stochastic-volatility-symmetry-volume-preservation.tex <==
\begin{table*}[t!]
    \centering
    \tiny
    \begin{tabular}{l|rrrrrr|rr|rr}
\toprule
       &&&&&&& \multicolumn{2}{c}{Volume Preservation} & \multicolumn{2}{c}{Symmetry} \\
    Method   & Acc. Prob. & Time (Sec.) &   Mean ESS &    Min. ESS &  \begin{tabular}[c]{@{}l@{}}Mean ESS \\ (Sec.)\end{tabular} &  \begin{tabular}[c]{@{}l@{}}Min. ESS \\ (Sec.)\end{tabular} & Median &    $90^\mathrm{th}$-Per. &  Median &    $90^\mathrm{th}$-Per. \\
\midrule
G.L.F.(a) & $0.78 \pm 0.0$ & $2616.70 \pm 16.5$ & $294.51 \pm 10.7$ & $121.79 \pm 7.7$ & $0.11 \pm 0.0$ & $0.05 \pm 0.0$ & $7.2\mathrm{e-}07$ & $3.1\mathrm{e-}06$ & $4.9\mathrm{e-}06$ & $2.5\mathrm{e-}05$ \\
G.L.F.(b) & $0.78 \pm 0.0$ & $2339.78 \pm 9.5$ & $297.82 \pm 9.2$ & $132.79 \pm 6.6$ & $0.13 \pm 0.0$ & $0.06 \pm 0.0$ & $6.7\mathrm{e-}07$ & $2.8\mathrm{e-}06$ & $5.0\mathrm{e-}06$ & $2.4\mathrm{e-}05$ \\
I.M.(a) & $0.80 \pm 0.0$ & $2761.61 \pm 8.3$ & $309.10 \pm 10.5$ & $133.32 \pm 7.8$ & $0.11 \pm 0.0$ & $0.05 \pm 0.0$ & $8.7\mathrm{e-}08$ & $2.2\mathrm{e-}07$ & $1.3\mathrm{e-}06$ & $2.4\mathrm{e-}06$ \\
I.M.(b) & $0.80 \pm 0.0$ & $2710.47 \pm 8.4$ & $296.72 \pm 9.2$ & $127.35 \pm 7.3$ & $0.11 \pm 0.0$ & $0.05 \pm 0.0$ & $1.7\mathrm{e-}07$ & $4.5\mathrm{e-}07$ & $2.8\mathrm{e-}06$ & $4.7\mathrm{e-}06$ \\
\bottomrule
\end{tabular}
    \caption{Comparison of the implicit midpoint generalized leapfrog integrators on the stochastic volatility model. We see that the implicit midpoint integrator is competitive on the effective sample size and timing comparisons. We also evaluate the median reversibility and volume preservation of the implicit midpoint and the generalized leapfrog integrators on the stochastic volatility model with $\delta = 1\times10^{-6}$. Here we see that the implicit midpoint integrator enjoys better conservation of volume and reversibility.}
    \label{tab:stochastic-volatility-symmetry-volume-preservation}
\end{table*}
